Egocentric Whole-Body Motion Capture with FisheyeViT and Diffusion-Based Motion Refinement

In this work, we explore egocentric whole-body motion capture using a single fisheye camera, which simultaneously estimates human body and hand motion. This task presents significant challenges due to three factors: the lack of high-quality datasets, fisheye camera distortion, and human body self-occlusion. To address these challenges, we propose a novel approach that leverages FisheyeViT to extract fisheye image features, which are subsequently converted into pixel-aligned 3D heatmap representations for 3D human body pose prediction. For hand tracking, we incorporate dedicated hand detection and hand pose estimation networks for regressing 3D hand poses. Finally, we develop a diffusion-based whole-body motion prior model to refine the estimated whole-body motion while accounting for joint uncertainties. To train these networks, we collect a large synthetic dataset, EgoWholeBody, comprising 840,000 high-quality egocentric images captured across a diverse range of whole-body motion sequences. Quantitative and qualitative evaluations demonstrate the effectiveness of our method in producing high-quality whole-body motion estimates from a single egocentric camera.

==> sec/bak/1_intro_bak.tex <==
\section{Introduction}
The rise of extended reality technologies, such as VR/AR/MR devices, has recently fueled the need for egocentric 3D human motion capture from head-mounted or body-mounted devices. This technology allows for the precise tracking and analysis of an individual's movements from their own perspective, offering an immersive user experience. A number of egocentric human body pose estimation works have been proposed, including Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}, GlobalEgoMocap~\cite{wang2021estimating}, EgoPW~\cite{Wang_2022_CVPR}, EgoHMR~\cite{liu2023egohmr} and SceneEgo~\cite{Wang_2022_CVPR}. These methods have made substantial advancements in this field. However, none of these works explored the whole-body pose estimation task, which limits the understanding of human activity and human-object interactions from the egocentric setting. Moreover, current methods still suffer from serious human body self-occlusion problems and they do not address the fisheye camera distortion effect explicitly.
%
% Egocentric pose estimation also holds the potential to change the way we interact with the virtual environment, making it a pivotal tool in human-computer interactions. 
%
% \ZC{I suggest making the motivation for egocentric pose estimation more concise, and should motivate more about the task of whole-body pose estimation, why we are interested in that, and why it is so challenging.}

To address this problem, we propose a new method that aims to capture the 3D \textit{whole-body} motion, including the human body and hand motion, through a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}).

% Our work focuses on capturing the 3D \textit{whole-body} motion, including the human body and hand motion, through a single head-mounted fisheye camera, which is illustrated in Fig.~\ref{fig:teaser}. 

% Our work focuses on capturing the 3D \textit{whole-body} motion, including the human body and hand motion, through a single head-mounted fisheye camera, which is illustrated in Fig.~\ref{fig:teaser}.  Notably, we do not consider facial expression estimation, as the face is often only partially visible in the egocentric perspective. \DL{I suggest to not mention this here; I would focus on saying that others did not predict hands, but hands are important, so we do.} A number of egocentric human body pose estimation works have been proposed, including Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}, GlobalEgoMocap~\cite{wang2021estimating}, EgoPW~\cite{Wang_2022_CVPR}, EgoHMR~\cite{liu2023egohmr} and SceneEgo~\cite{Wang_2022_CVPR}. These methods have made substantial advancements in the field of egocentric pose estimation. However, none of these works explored the whole-body pose estimation task, which limits the understanding of human activity and human-object interactions from the egocentric setting. Moreover, current methods still suffer from the fisheye camera distortion effect and serious human body self-occlusion problems. 


\ZC{There is a large discontinuity in the flow, while the last paragraph talks about the limitations of previous methods, this paragraph starts to sell the new dataset. I suggest proposing our method first in the following paragraphs and describe how we address the above mentioned issues, then we can motivate the dataset like, "To train such a system, we requires training data with GT annotations for both body and hand pose. However, none of previous datasets have that ..."} Though many training datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d} for egocentric body pose estimation have been proposed, the dataset for whole-body motion capture is still absent. To solve this, we introduce a large-scale high-quality synthetic dataset named \textit{EgoWholeMocap}. 
% As there is currently no existing dataset suitable for egocentric whole-body pose estimation, we introduce a large-scale high-quality synthetic dataset named \textit{EgoWholeMocap}. 
The EgoWholeMocap dataset contains over 870k frames and covers large varieties of whole-body motion. To generate this synthetic dataset, we drive the rigged renderpeople models~\cite{renderpeople} and SMPL-X model~\cite{pavlakos2019expressive} with mixamo motion sequences~\cite{mixamo}, which feature diverse human body movements. Additionally, the dataset incorporates hand motion data from the GRAB~\cite{taheri2020grab} and TCDHands~\cite{hoyet2012sleight} motion sequences to present diverse hand movements.

Next, we present a novel single-frame egocentric whole-body pose estimation method to effectively tackle the challenge of fisheye camera distortion. We recognize that attempting to undistort the entire egocentric view is impractical due to the large field of view (FOV) of the fisheye lens. However, we devise a practical solution by partitioning the image into smaller patches, with each patch aligning with a specific FOV range, which can then be individually undistorted. These undistorted patches are subsequently fed into a transformer network to extract image features. We call this framework ``FisheyeViT'' for its capacity to address the distortion of fisheye images. 

Following the extraction of image features, our approach converts these features into 3D heatmap representations for regressing 3D body joints. However, the 3D heatmap representations in existing methods, such as Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} and Sun~\etal's work~\cite{sun2018integral}, rely on the assumption of a weak-perspective camera model, which is different from the highly-distorted egocentric camera model. To solve this problem, we let the network learn a \textit{pixel-aligned 3D heatmap} representation that aligns with the egocentric image features. The joint locations from the pixel-aligned heatmap are further transformed with the fisheye camera model to obtain the final 3D body pose. We also train a hand detection network and a 3D hand pose estimation network to obtain 3D hand poses from a single image. \ZC{this paragraph describes the body pose estimation and hand pose estimation as two separate methods, is there anything can be used in common, like feature map? We should probably discuss the difficulty of estimating the body hand pose in a single network due to the resolution, memory constraints, etc., then we train another network specifically for the hand. They are later fused in the diffusion refinement stage. }

To effectively address the self-occlusion challenge and elevate the accuracy of our method, we introduce a new strategy that harnesses the temporal context and whole-body motion priors for refining 3D body and hand motion estimations. Specifically, we design an uncertainty-aware diffusion-based motion refinement strategy. This approach refines the motion by considering the uncertainty associated with each joint. It retains joints with low uncertainty while allowing the whole-body diffusion model to generate joints with high uncertainty, conditioned upon the information from the low-uncertainty joints. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. \ZC{perhaps talk more benefits of using one joint diffusion model for hand and body because the hand module and body module are quite isolated explained in my previous comment. One benefit I can think about is the diffusion model can improve the motion prediction by learning the correlation between hand motion and body motion from datasets.}

% In order to deal with the self-occlusion issue and further enhance the quality of estimated poses, we leverage the temporal context and whole-body motion prior to refine the estimated 3D body and hand motion. We develop an uncertainty-aware diffusion-based motion refinement strategy to refine the motion considering the uncertainty of each joint: we keep the joints with low uncertainty and let the whole-body diffusion model generate the joints with high uncertainty conditioned on the low-uncertainty joints.

We evaluate our estimated human body poses across a range of datasets, including SceneEgo~\cite{wang2023scene}, GlobalEgoMocap~\cite{wang2021estimating} and Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}. Furthermore, we employ a multi-view mocap system to capture the ground truth hand motion of the SceneEgo dataset~\cite{wang2023scene} and evaluate the accuracy of estimated hand poses on this dataset. Our approaches, both the single-frame method and the diffusion-based refinement method, consistently outperform all baseline methods both qualitatively and quantitatively. To summarize, our contributions are listed as follows:

\begin{itemize}
    \item The first egocentric whole-body motion capture framework that predicts accurate and temporarily coherent egocentric body and hand motion;
    \item EgoWholeMocap, a new high-quality synthetic dataset for egocentric whole-body motion capture;
    \item FisheyeViT for alleviating fisheye camera distortion and pixel-aligned 3D heatmap representation for accurate egocentric body pose estimation from a single image;
    % \item By leveraging whole-body motion diffusion models and a confidence-aware refining process, our method corrects initial motion estimations and significantly outperforms previous approaches. \DL{In this contribution I would emphasize that the proposed confidence-aware diffusion model helps to predict plausible whole-body motion even under occlusion, which is a constant issue in egocentric pose estimation. SOTA results you can skip to after the bullets, as a consequence of our contribution.}
    \item By leveraging whole-body motion diffusion models and a confidence-aware refining process, our method corrects initial estimations and predicts plausible whole-body motions even under occlusion, which is a persistent challenge in egocentric pose estimation.
\end{itemize}

As a consequence of our contributions, our method has shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This emphasizes the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. \ZC{perhaps delete this paragraph and merge the part into the paragraph before the listed contributions}

==> sec/bak/1_intro_bak2.tex <==
\section{Introduction}
The rise of extended reality technologies, such as VR/AR/MR devices, has recently fueled the need for egocentric 3D human motion capture from head-mounted or body-mounted devices. This technology allows for the precise tracking and analysis of individual's movements from their own perspective, offering an immersive user experience. A number of egocentric human body pose estimation works have made substantial advancements in this field, including Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}, GlobalEgoMocap~\cite{wang2021estimating}, EgoPW~\cite{Wang_2022_CVPR}, EgoHMR~\cite{liu2023egohmr} and SceneEgo~\cite{Wang_2022_CVPR}. However, none of these works explored the whole-body pose estimation task, which limits the understanding of human activity and human-object interactions from the egocentric setup. Moreover, current methods still suffer from serious human body self-occlusion problems and the fisheye camera distortion issue. 
% \ZC{I suggest making the motivation for egocentric pose estimation more concise, and should motivate more about the task of whole-body pose estimation, why we are interested in that, and why it is so challenging.}

To address these problems, we propose a new method that aims to capture 3D \textit{whole-body} motions, including human body and hand motions, using a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}). We first present a novel single-frame egocentric whole-body pose estimation method to effectively tackle the challenge of fisheye camera distortion. We found that undistorting the entire egocentric view is impractical due to the large field of view (FOV) of the fisheye lens. However, we devise a practical solution by partitioning the image into smaller patches, with all patches aligning with a specific FOV range, which can then be individually undistorted. These undistorted patches are subsequently fed into a transformer network to extract image features. We call this framework ``\emph{FisheyeViT}'' for its ability to address the distortion issue of fisheye images. 

Following the extraction of image features, our approach converts these features into 3D heatmap representations for regressing 3D body joints. However, the 3D heatmap representations in existing methods, such as Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} and Sun~\etal's work~\cite{sun2018integral}, rely on the assumption of a weak perspective camera model, which is different from the highly-distorted egocentric camera model. To solve this, we learn a \emph{pixel-aligned 3D heatmap} representation that aligns with the egocentric image features. The joint locations from the pixel-aligned heatmap are further transformed with the fisheye camera model to get the final 3D poses. 

Due to the wide range of hand sizes in the egocentric camera perspective, we train a separate hand detection network to extract undistorted hand images. We further introduce a hand pose estimation network to regress 3D hand poses from cropped hand images. 
% \ZC{this paragraph describes the body pose estimation and hand pose estimation as two separate methods, is there anything can be used in common, like feature map? We should probably discuss the difficulty of estimating the body hand pose in a single network due to the resolution, memory constraints, etc., then we train another network specifically for the hand. They are later fused in the diffusion refinement stage. }

To address the self-occlusion challenge and improve the accuracy of our method, we introduce a new whole-body motion refinement method that harnesses the temporal context and whole-body motion priors. We first train a diffusion model to learn the whole-body motion prior, encoding the correlation between hand and body motion. Next, we design an uncertainty-aware diffusion-based motion refinement strategy to refine the motion by considering the uncertainty associated with each joint. It retains joints with low uncertainty while allowing the whole-body diffusion model to generate joints with high uncertainty, conditioned on the information from the low-uncertainty joints. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. 
% To effectively address the self-occlusion challenge and elevate the accuracy of our method, we introduce a new strategy that harnesses the temporal context and whole-body motion priors for refining 3D body and hand motion estimations. Specifically, we design an uncertainty-aware diffusion-based motion refinement strategy. This approach refines the motion by considering the uncertainty associated with each joint. It retains joints with low uncertainty while allowing the whole-body diffusion model to generate joints with high uncertainty, conditioned upon the information from the low-uncertainty joints. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. \ZC{perhaps talk more benefits of using one joint diffusion model for hand and body because the hand module and body module are quite isolated explained in my previous comment. One benefit I can think about is the diffusion model can improve the motion prediction by learning the correlation between hand motion and body motion from datasets.}

% \ZC{There is a large discontinuity in the flow, while the last paragraph talks about the limitations of previous methods, this paragraph starts to sell the new dataset. I suggest proposing our method first in the following paragraphs and describe how we address the above mentioned issues, then we can motivate the dataset like, "To train such a system, we requires training data with GT annotations for both body and hand pose. However, none of previous datasets have that ..."} 
Training our method requires large-scale training data with ground truth annotations for both body and hand poses. However, such data are absent in all existing  datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d}. To solve this, we introduce a new large-scale high-quality synthetic dataset named \emph{EgoWholeMocap}. The EgoWholeMocap dataset contains over 870k frames and covers diverse whole-body motions. To generate this synthetic dataset, we drive the rigged renderpeople models~\cite{renderpeople} and SMPL-X model~\cite{pavlakos2019expressive} with mixamo motion sequences~\cite{mixamo} that contain large-scale diverse human body movements. Additionally, the dataset incorporates hand motion data from the GRAB~\cite{taheri2020grab} and TCDHands~\cite{hoyet2012sleight} sequences to present diverse hand motions.

We evaluate our estimated human body poses across a range of datasets, including SceneEgo~\cite{wang2023scene}, GlobalEgoMocap~\cite{wang2021estimating} and Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}. Furthermore, we employ a multi-view mocap system to capture the ground truth hand motion of the SceneEgo dataset~\cite{wang2023scene} and evaluate the accuracy of estimated hand poses on this dataset. 
% Our approaches, both the single-frame method and the diffusion-based refinement method, consistently outperform all baseline methods both qualitatively and quantitatively. To summarize, our contributions are listed as follows:
Our approaches
% , both the single-frame method and the diffusion-based refinement method \LJ{do we need to mention two settings of our method here? Can we just  say "Our approach"? }, 
have shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This demonstrates the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. In summary, we have the following contributions:

\begin{itemize}
    \item The first egocentric whole-body motion capture framework that predicts accurate and temporarily coherent egocentric body and hand motion;
    \item EgoWholeMocap, a new high-quality synthetic dataset for egocentric whole-body motion capture;
    \item FisheyeViT for alleviating fisheye camera distortion and pixel-aligned 3D heatmap representation for accurate egocentric body pose estimation from a single image;
    % \item By leveraging whole-body motion diffusion models and a confidence-aware refining process, our method corrects initial motion estimations and significantly outperforms previous approaches. \DL{In this contribution I would emphasize that the proposed confidence-aware diffusion model helps to predict plausible whole-body motion even under occlusion, which is a constant issue in egocentric pose estimation. SOTA results you can skip to after the bullets, as a consequence of our contribution.}
    \item Uncertainty-aware refining network based on motion diffusion models, to correct initial pose estimations and to predict plausible motions even under occlusion.
\end{itemize}

% As a consequence of our contributions, our method has shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This emphasizes the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. \ZC{perhaps delete this paragraph and merge the part into the paragraph before the listed contributions}

==> sec/bak/1_intro_bak3.tex <==
\section{Introduction}
Egocentric 3D human motion estimation using head-mounted devices~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19} has garnered significant traction in recent years, driven by its diverse applications in VR/AR. Immersed in a virtual world, we can traverse virtual environments, interact with virtual objects, and even simulate real-world interactions. To fully capture the intricacies of human motion during such interaction, understanding both body and hand movements is essential. While existing egocentric motion capture methods~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19, wang2021estimating, Wang_2022_CVPR, liu2023egohmr, wang2023scene} focus solely on body motion, neglecting the hands, this work proposes the task of egocentric \emph{whole-body} motion estimation, i.e., simultaneous estimation of the body motion and hand motion from a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}). This task is extremely challenging due to three factors. \JW{add another challenge about dataset. no available dataset...}
%The emergence of extended reality technologies, such as VR/AR/MR devices, has recently fueled the need for capturing whole-body motion, \ie human body and hand motions, from the down-facing fisheye camera on the head-mounted device~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19}. This task is essential for creating immersive virtual experiences, enhancing gaming realism, supporting behavioral research, and aiding in medical recovery. However, tackling this task is tough due to three main challenges. 
First, the fisheye image introduces significant distortion, making it difficult for existing networks, which are designed for non-distorted images, to extract features. Second, the large size difference between the human body and hands makes it difficult to simultaneously capture both. Third, the human body is frequently occluded in the egocentric camera perspective.
%Existing egocentric motion capture methods~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19, wang2021estimating, Wang_2022_CVPR, liu2023egohmr, wang2023scene} only focus on human body poses, while omitting the hands, and they still suffer from the fisheye camera distortion and occlusion issues.


% \todo{\textbf{Old:} The rise of extended reality technologies, such as VR/AR/MR devices, has recently fueled the need for egocentric 3D human motion capture from head-mounted or body-mounted devices. This technology allows for the precise tracking and analysis of individual's movements from their own perspective, offering an immersive user experience. A number of egocentric human body pose estimation works have made substantial advancements in this field, including Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}, GlobalEgoMocap~\cite{wang2021estimating}, EgoPW~\cite{Wang_2022_CVPR}, EgoHMR~\cite{liu2023egohmr} and SceneEgo~\cite{Wang_2022_CVPR}. However, none of these works explored the whole-body pose estimation task, which limits the understanding of human activity and human-object interactions from the egocentric setup. Moreover, current methods still suffer from serious human body self-occlusion problems and the fisheye camera distortion issue. }

%To address these challenges, we propose a new method that aims to capture 3D \textit{whole-body} motions, including human body and hand motions, using a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}). 

\JW{Firstly say we split the hand pose and body pose estimation.  For the hand pose estimation, we ...... (simple explanation).}
\ZC{need to make the following few method paragraphs more concise, discuss more about the insights, and improvements instead of covering a lot of method details}
To address these challenges, we first present a novel single-frame \JW{Do not say single frame here.} egocentric whole-body pose estimation method to tackle the challenge of fisheye camera distortion effectively. We found that undistorting the entire egocentric view is impractical due to the large field of view (FOV) of the fisheye lens. However, we devise a practical solution by partitioning the image into smaller patches, with all patches aligning with a specific FOV range, which can then be individually undistorted. These undistorted patches are subsequently fed into a transformer network to extract image features. We call this framework ``\emph{FisheyeViT}'' for its ability to address the distortion issue of fisheye images. 

\JW{Another issue introduced by the Fisheye distortion...}
Following the extraction of image features, our approach converts these features into 3D heatmap representations for regressing 3D body joints. However, the 3D heatmap representations in existing methods, such as Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} and Sun~\etal's work~\cite{sun2018integral}, rely on the assumption of a weak perspective camera model, which is different from the highly-distorted egocentric camera model. \JW{} To solve this, we learn a \emph{pixel-aligned 3D heatmap} representation that aligns with the egocentric image features. The joint locations from the pixel-aligned heatmap are further transformed with the fisheye camera model to get the final 3D poses. 

Due to the wide range of hand sizes in the egocentric camera perspective, we train a separate hand detection network to extract undistorted hand images. We further introduce a hand pose estimation network to regress 3D hand poses from cropped hand images. 

\JW{repetition, where does the uncertainty come from}
\JW{if we have a temporal sequence}
To address the self-occlusion challenge and improve the accuracy of our method, we introduce a new whole-body motion refinement method that harnesses the temporal context and whole-body motion priors. We first train a diffusion model to learn the whole-body motion prior, encoding the correlation between hand and body motion. Next, we design an uncertainty-aware \JW{where does uncertainty comes from} diffusion-based motion refinement strategy to refine the motion by considering the uncertainty associated with each joint. It retains joints with low uncertainty while allowing the whole-body diffusion model to generate joints with high uncertainty, conditioned on the information from the low-uncertainty joints. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. 

Training our method requires large-scale training data with ground truth annotations for both body and hand poses. However, such data are absent in all existing  datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d}. To solve this, we introduce a new large-scale high-quality synthetic dataset named \emph{EgoWholeMocap}. Our EgoWholeMocap dataset contains over 870k frames and covers diverse whole-body motions. 
% To generate this synthetic dataset, we drive the rigged renderpeople models~\cite{renderpeople} and SMPL-X model~\cite{pavlakos2019expressive} with mixamo motion sequences~\cite{mixamo} that contain large-scale diverse human body movements. Additionally, the dataset incorporates hand motion data from the GRAB~\cite{taheri2020grab} and TCDHands~\cite{hoyet2012sleight} sequences to present diverse hand motions.
The EgoWholeMocap dataset is larger than previous egocentric training datasets, providing a valuable resource for advancing research in egocentric whole-body motion capture. 

We evaluate our estimated human body poses across a range of datasets, including SceneEgo~\cite{wang2023scene}, GlobalEgoMocap~\cite{wang2021estimating} and Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}. Furthermore, we employ a multi-view mocap system to capture the ground truth hand motion of the SceneEgo dataset~\cite{wang2023scene} and evaluate the accuracy of estimated hand poses on this dataset. Our approaches have shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. 
\ZC{Add discussion of the in-the-wild results, because this could be impressive point} 
This demonstrates the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. In summary, we have the following contributions:

\begin{itemize}
    \item The first egocentric whole-body motion capture method that predicts accurate and temporarily coherent egocentric body and hand motion;
    \item FisheyeViT for alleviating fisheye camera distortion and pixel-aligned 3D heatmap representation for accurate egocentric body pose estimation from a single image;
    % \item By leveraging whole-body motion diffusion models and a confidence-aware refining process, our method corrects initial motion estimations and significantly outperforms previous approaches. \DL{In this contribution I would emphasize that the proposed confidence-aware diffusion model helps to predict plausible whole-body motion even under occlusion, which is a constant issue in egocentric pose estimation. SOTA results you can skip to after the bullets, as a consequence of our contribution.}
    \item Uncertainty-aware refining method based on motion diffusion models for correcting initial pose estimations and predicting plausible motions even under occlusion;
    \item EgoWholeMocap, a new high-quality synthetic dataset for egocentric whole-body motion capture.
\end{itemize}

% As a consequence of our contributions, our method has shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This emphasizes the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. \ZC{perhaps delete this paragraph and merge the part into the paragraph before the listed contributions}

==> sec/bak/1_intro_bak4.tex <==
\section{Introduction}
Egocentric 3D human motion estimation using head-mounted devices~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19} has garnered significant traction in recent years, driven by its diverse applications in VR/AR. Immersed in a virtual world, we can traverse virtual environments, interact with virtual objects, and even simulate real-world interactions. To fully capture the intricacies of human motion during such interaction, understanding both body and hand movements is essential. While existing egocentric motion capture methods~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19, wang2021estimating, Wang_2022_CVPR, liu2023egohmr, wang2023scene} focus solely on body motion, neglecting the hands, this work proposes the task of egocentric \emph{whole-body} motion capture, \ie simultaneous estimation of the body motion and hand motion from a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}). This task is extremely challenging due to three factors. 
%First, the fisheye image introduces significant distortion, making it difficult for existing networks, which are designed for non-distorted images, to extract features. Second, the large size difference between the human body and hands makes it difficult to simultaneously capture both. Third, the human body is frequently occluded in the egocentric camera perspective. Last, large-scale training data with ground truth annotations for both body and hand poses is absent in existing datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d}.
First, the fisheye image introduces significant distortion, making it difficult for existing networks, which are designed for non-distorted images, to extract features. Second, the egocentric camera perspective frequently leads to occlusion of body parts, particularly the hands, further complicating the task of whole-body motion capture. Last, large-scale training data with ground truth annotations for both body and hand poses is absent in existing datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d}.

% \todo{\textbf{Old:} The rise of extended reality technologies, such as VR/AR/MR devices, has recently fueled the need for egocentric 3D human motion capture from head-mounted or body-mounted devices. This technology allows for the precise tracking and analysis of individual's movements from their own perspective, offering an immersive user experience. A number of egocentric human body pose estimation works have made substantial advancements in this field, including Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19}, GlobalEgoMocap~\cite{wang2021estimating}, EgoPW~\cite{Wang_2022_CVPR}, EgoHMR~\cite{liu2023egohmr} and SceneEgo~\cite{Wang_2022_CVPR}. However, none of these works explored the whole-body pose estimation task, which limits the understanding of human activity and human-object interactions from the egocentric setup. Moreover, current methods still suffer from serious human body self-occlusion problems and the fisheye camera distortion issue. }

%To address these challenges, we propose a new method that aims to capture 3D \textit{whole-body} motions, including human body and hand motions, using a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}). 

% \JW{Firstly say we split the hand pose and body pose estimation.  For the hand pose estimation, we ...... (simple explanation).}
%In this work, we propose a new egocentric whole-body motion capture method to address these challenges. To address the fisheye distortion challenge, we introduce \emph{FisheyeViT} and \emph{pixel-aligned 3D heatmap} to regress human body poses from a single frame. Note that undistorting the entire egocentric view is impractical due to the large field of view (FOV) of the fisheye lens, we use the \emph{FisheyeViT} network to first partition the image into smaller patches, with all patches aligning with a specific FOV range, which can then be individually undistorted. These undistorted patches are subsequently fed into a transformer network to extract image features. The extracted features are converted into 3D heatmap representations for regressing 3D body joints. However, existing 3D heatmap representation for egocentric pose estimation~\cite{wang2023scene} reprojects the image features into 3D space with the complex fisheye reprojection function, making it difficult to learn the correlation between 3D human pose and 2D features. To solve this, we learn a \emph{pixel-aligned 3D heatmap} representation, where voxels in the 3D heatmap directly correspond to the pixels in 2D image features. The joint locations from the pixel-aligned heatmap are further transformed with the fisheye camera model to get the final 3D human body poses. 

In this work, we propose a novel egocentric whole-body motion capture method to address the above-mentioned challenges. To effectively tackle fisheye distortion, we introduce the \emph{FisheyeViT} and pixel-aligned 3D heatmap for regressing 3D human poses. Instead of attempting to undistort the entire fisheye image, which is impractical due to the fisheye lens's large field of view (FOV), we partition the image into smaller patches aligned with specific FOV ranges. This facilitates individual patch-level undistortion and aligns well with the vision transformer architecture which we employ to extract the full image feature map from these patches. We name our approach \emph{FisheyeViT}. We further utilize 3D heatmap representations for 3D body joint regression due to their ability to preserve joint uncertainties. Unlike existing 3D heatmap representations~\cite{wang2023scene} that reproject image features into 3D space using complex fisheye reprojection function, our pixel-aligned 3D heatmap representation directly corresponds voxels in the 3D heatmap to pixels in the 2D image features, simplifying the learning process. \ZC{still hard to understand the difference} Finally, joint locations from the pixel-aligned heatmap are transformed with the fisheye camera model to obtain the final 3D human body poses. \JW{write the process of getting the 3d heatmap. previous: use complex fisheye re-projection function to get 3D heatmap. Ours: directly use simple de-conv layers to get.}


Due to the large size differences between the body and hands, the resolution of hands may be significantly reduced in the down-sampled network input. To solve this, we introduce a hand detection network to extract high-resolution, undistorted hand images from the original egocentric image. We further train a hand pose estimation network to accurately regress 3D hand poses. \JW{due to large..., we train separate network...}

To address the challenge of self-occlusion and enhance pose estimation accuracy, we introduce a novel method for refining whole-body motion by leveraging temporal context and motion prior. We first train a diffusion model to learn the whole-body motion prior, encoding the correlation between hand and body movements. Subsequently, we extract the joint uncertainties from the pixel-aligned 3D heatmap and refine the whole-body motion under the uncertainty guidance. This involves retaining joints with low uncertainty while enabling the whole-body diffusion model to generate joints with high uncertainty, conditioned on the low-uncertainty joints. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. 

In response to the absence of the egocentric whole-body motion capture datasets, we introduce a new large-scale high-quality synthetic dataset named \emph{EgoWholeMocap}. Comprising over 870k frames, this dataset encompasses a wide range of whole-body motions. Significantly surpassing the size of previous egocentric training datasets, EgoWholeMocap serves as a valuable resource for advancing research in egocentric whole-body motion capture.

%\todo{This is another version of introduction.}
%\JW{In this work, we propose a new egocentric whole-body motion capture method to address these challenges. We first use the \emph{FisheyeViT} and \emph{pixel-aligned 3D heatmap} to regress the human body from a single image. Then we train a separate hand detection and pose estimation network to get 3D hand poses. Finally, we refine the whole-body motion using a diffusion-based uncertainty-aware method.}

%\JW{We first introduce \emph{FisheyeViT} network to extract egocentric image features. Note that undistorting the entire egocentric view is impractical due to the large field of view (FOV) of the fisheye lens, we first partition the image into smaller patches, with all patches aligning with a specific FOV range, which can then be individually undistorted. These undistorted patches are subsequently fed into a transformer network to extract image features. The features are converted into the \emph{pixel-aligned 3D heatmap} representations for regressing 3D body joints. The \emph{pixel-aligned 3D heatmap} is specially designed for the egocentric pose estimation task under the fisheye camera model, where voxels in the 3D heatmap directly correspond to the pixels in 2D image features. The joint locations from the pixel-aligned heatmap are further transformed with the fisheye camera model to get the final 3D poses. }

%\JW{We further enhance the accuracy of our predicted single-frame poses with an uncertainty-aware motion refinement strategy. We first train a diffusion model to learn the whole-body motion prior, encoding the correlation between hand and body motion. Next, we obtain the joint uncertainties from the pixel-aligned 3D heatmap and refine the whole-body motion under the uncertainty guidance. High-uncertainty joint positions are generated with the diffusion model conditioned on the low-uncertainty joint positions. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. }

%\JW{To train our whole-body pose estimation networks, we introduce a new large-scale high-quality synthetic dataset named \emph{EgoWholeMocap}. Our EgoWholeMocap dataset contains over 870k frames and covers diverse whole-body motions. The EgoWholeMocap dataset is larger than previous egocentric training datasets, providing a valuable resource for advancing research in egocentric whole-body motion capture. }

We evaluate our estimated human body poses across a range of datasets, including SceneEgo~\cite{wang2023scene}, GlobalEgoMocap~\cite{wang2021estimating} and Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}. Furthermore, we employ a multi-view mocap system to capture the ground truth hand motion of the SceneEgo dataset~\cite{wang2023scene} and evaluate the accuracy of estimated hand poses on this dataset. Our approaches have shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This demonstrates the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. In summary, we have the following contributions:

\begin{itemize}
    \item The first egocentric whole-body motion capture method that predicts accurate and temporarily coherent egocentric body and hand motion;
    \item FisheyeViT for alleviating fisheye camera distortion and pixel-aligned 3D heatmap representation for accurate egocentric body pose estimation from a single image;
    % \item By leveraging whole-body motion diffusion models and a confidence-aware refining process, our method corrects initial motion estimations and significantly outperforms previous approaches. \DL{In this contribution I would emphasize that the proposed confidence-aware diffusion model helps to predict plausible whole-body motion even under occlusion, which is a constant issue in egocentric pose estimation. SOTA results you can skip to after the bullets, as a consequence of our contribution.}
    \item Uncertainty-aware refining method based on motion diffusion models for correcting initial pose estimations and predicting plausible motions even under occlusion;
    \item EgoWholeMocap, a new high-quality synthetic dataset for egocentric whole-body motion capture.
\end{itemize}

% As a consequence of our contributions, our method has shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This emphasizes the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. \ZC{perhaps delete this paragraph and merge the part into the paragraph before the listed contributions}

==> sec/bak/1_intro_bak_diogo.tex <==
\section{Introduction}
Egocentric 3D human motion estimation using head-mounted devices~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19} has garnered significant traction in recent years, driven by its diverse applications in VR/AR. Immersed in a virtual world, we can traverse virtual environments, interact with virtual objects, and even simulate real-world interactions. To fully capture the intricacies of human motion during such interaction, understanding both body and hand movements is essential. While existing egocentric motion capture methods~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19, wang2021estimating, Wang_2022_CVPR, liu2023egohmr, wang2023scene} focus solely on body motion, neglecting the hands, this work proposes the task of egocentric \emph{whole-body} motion capture, \ie simultaneous estimation of the body motion and hand motion from a single head-mounted fisheye camera (shown in Fig.~\ref{fig:teaser}). This task is extremely challenging due to three factors. 
First, the fisheye image introduces significant distortion, making it difficult for existing networks, which are designed for non-distorted images, to extract features. Second, the egocentric camera perspective frequently leads to the occlusion of body parts, particularly the hands, further complicating the task of whole-body motion capture. Last, large-scale training data with ground truth annotations for both body and hand poses is absent in existing datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d}.

In this work, we propose a novel egocentric whole-body motion capture method to address the above challenges. To effectively tackle fisheye distortion, we introduce the \emph{FisheyeViT} and a joint regressor using \emph{pixel-aligned 3D heatmap} for predicting 3D human poses. Instead of attempting to undistort the entire fisheye image, which is impractical due to the fisheye lens's large field of view (FOV), we partition the image into smaller patches aligned with specific FOV ranges. This facilitates individual patch-level undistortion and aligns well with the vision transformer architecture which we employ to extract the full image feature map from these patches. 
We name this approach \emph{FisheyeViT}. 
We further propose an egocentric 3D pose regressor utilizing 3D heatmap representations due to their ability to preserve joint uncertainties. Unlike existing 3D heatmap-based egocentric pose regressor~\cite{wang2023scene} that reproject image features into 3D space using complex fisheye reprojection function, our egocentric pose regressor uses simple deconvolutional layers to get pixel-aligned 3D heatmap. The voxels in the 3D heatmap thus directly correspond to the pixels in 2D features, and further to image patches in FisheyeViT, which facilitates the network learning process. Joint locations from the pixel-aligned 3D heatmap are finally transformed with the fisheye camera model to obtain the 3D human body poses.
% pixel-aligned 3D heatmap representation directly corresponds voxels in the 3D heatmap to pixels in the 2D image features, simplifying the learning process. Finally, joint locations from the pixel-aligned heatmap are transformed with the fisheye camera model to obtain the final 3D human body poses. 
% \JW{write the process of getting the 3d heatmap. previous: use complex fisheye re-projection function to get 3D heatmap. Ours: directly use simple de-conv layers to get.}
Due to the large size differences between the body and hands, we train a hand detection network and a hand pose estimation network to accurately regress 3D hand poses.
% Due to the large size differences between the body and hands, we train a separate hand detection network to extract high-resolution, undistorted hand images and use a hand pose estimation network to accurately regress 3D hand poses.

% In this work, we propose a novel egocentric whole-body motion capture method to address the above-mentioned challenges. To effectively tackle fisheye distortion, we introduce the \emph{FisheyeViT} and a joint regressor using \emph{pixel-aligned 3D heatmap} for predicting 3D human poses. Instead of attempting to undistort the entire fisheye image, which is impractical due to the fisheye lens's large field of view (FOV), we partition the image into smaller patches aligned with specific FOV ranges. This facilitates individual patch-level undistortion and aligns well with the vision transformer architecture which we employ to extract the full image feature map from these patches. We name our approach \emph{FisheyeViT}. We further utilize 3D heatmap representations for 3D body joint regression due to their ability to preserve joint uncertainties. Unlike existing 3D heatmap-based egocentric pose regressor~\cite{wang2023scene} that reproject image features into 3D space using complex fisheye reprojection function, our egocentric pose regressor uses simple deconvolutional layers to directly get pixel-aligned 3D heatmap. Joint locations from the pixel-aligned heatmap are transformed with the fisheye camera model to obtain the final 3D human body poses pixel-aligned 3D heatmap representation directly corresponds voxels in the 3D heatmap to pixels in the 2D image features, simplifying the learning process. Finally, joint locations from the pixel-aligned heatmap are transformed with the fisheye camera model to obtain the final 3D human body poses. 
% \JW{write the process of getting the 3d heatmap. previous: use complex fisheye re-projection function to get 3D heatmap. Ours: directly use simple de-conv layers to get.}
% Due to the large size differences between the body and hands, we train a separate hand detection network to extract high-resolution, undistorted hand images and use a hand pose estimation network to accurately regress 3D hand poses.

% Due to the large size differences between the body and hands, the resolution of hands may be significantly reduced in the down-sampled network input. To solve this, we introduce a hand detection network to extract high-resolution, undistorted hand images from the original egocentric image. We further train a hand pose estimation network to accurately regress 3D hand poses. \JW{due to large..., we train separate network...}

To address the challenge of self-occlusion and enhance pose estimation accuracy, we introduce a novel method for refining whole-body motion by leveraging temporal context and motion prior. We first train a diffusion model to learn the whole-body motion prior, encoding the correlation between hand and body movements. Subsequently, we extract the joint uncertainties from the pixel-aligned 3D heatmap and refine the whole-body motion under the uncertainty guidance. This involves retaining joints with low uncertainty while enabling the whole-body diffusion model to generate joints with high uncertainty, conditioned on the low-uncertainty joints. This strategy significantly enhances the overall quality of our motion estimations, ensuring a more accurate and reliable outcome. 

In response to the absence of the egocentric whole-body motion capture datasets, we introduce a new large-scale high-quality synthetic dataset named \emph{EgoWholeMocap}. Comprising over 870k frames, this dataset encompasses a wide range of whole-body motions. Significantly surpassing the size of previous egocentric training datasets, EgoWholeMocap serves as a valuable resource for advancing research in egocentric whole-body motion capture.

We evaluate our estimated human body poses across a range of datasets, including SceneEgo~\cite{wang2023scene}, GlobalEgoMocap~\cite{wang2021estimating} and Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19}. Furthermore, we employ a multi-view mocap system to capture the ground truth hand motion of the SceneEgo dataset~\cite{wang2023scene} and evaluate the accuracy of estimated hand poses on this dataset. Our approaches have shown remarkable improvements in estimating egocentric whole-body motion compared to previous approaches. This demonstrates the effectiveness of our approach in addressing the special challenges in the egocentric view, including the fisheye distortion and self-occlusion. In summary, we have the following contributions:

\begin{itemize}
    \item The first egocentric whole-body motion capture method that predicts accurate and temporarily coherent egocentric body and hand motion;
    \item FisheyeViT for alleviating fisheye camera distortion and pose regressor using pixel-aligned 3D heatmap for accurate egocentric body pose estimation from a single image;
    \item Uncertainty-aware refining method based on motion diffusion models for correcting initial pose estimations and predicting plausible motions even under occlusion;
    \item EgoWholeMocap, a new high-quality synthetic dataset for egocentric whole-body motion capture.
\end{itemize}


==> sec/bak/3_method_bak.tex <==
\section{Method} \label{method}
We propose a new method for predicting accurate egocentric whole-body poses from egocentric image sequences. An overview of our approach is shown in Fig.~\ref{fig:framework}. We first generate a new large-scale synthetic dataset called EgoWholeMocap (Sec.~\ref{method:synthetic_dataset}). Based on this dataset, we propose a single-frame whole-body pose estimation method including three components: the FisheyeViT (Sec.~\ref{method:fisheyevit}) for extracting egocentric image features; the pixel-aligned 3D heatmap (Sec.~\ref{method:pixel_aligned_heatmap}) for further obtaining 3D body poses; the hand pose estimator (Sec.~\ref{method:wholebodypose}) for regressing 3D hand poses. Finally, we refine the combined human hand and body motion with the uncertainty-aware diffusion model (Sec.~\ref{method:diffusion}). \DL{A general comment is that we already mention a quite detailed overview of all the steps in the method back in the introduction; then we mention it here again in a more high level. I think that, if we already mention an overview in the intro L040-L097, we can skip it here;}
% We propose a new method for predicting accurate egocentric whole-body poses from egocentric image sequences. An overview of our approach is shown in Fig.~\ref{fig:framework}. We first generate a new large-scale synthetic dataset called EgoFullBody (Sec.~\ref{method:synthetic_dataset}). Based on this dataset, we train the FisheyeViT (Sec.~\ref{method:fisheyevit}) to extract egocentric image features, which are encoded with the pixel-aligned heatmap (Sec.~\ref{method:pixel_aligned_heatmap}) to further obtain the 3D body pose. Next, the hand image is cropped with the hand detection network and sent to the hand pose estimation network to regress 3D hand poses (Sec.~\ref{method:wholebodypose}). Finally, we refine the combined human hand and body motion with the uncertainty-aware diffusion model (Sec.~\ref{method:diffusion}).

\subsection{EgoWholeMocap Dataset} \label{method:synthetic_dataset}
\JW{Firstly motivate why hands, . 
Then analysis why estimating whole body is challenging. 
then refer to existing methods}
% Though many training datasets~\cite{akada2022unrealego,DBLP:journals/tvcg/XuCZRFST19,DBLP:conf/iccv/TomePAB19,Wang_2022_CVPR,liu2023egofish3d} for egocentric body pose estimation have been proposed, the dataset for whole-body motion capture is still absent.
% \DL{this sentence would be better in the intro or in the RW}
In this section, we propose EgoWholeMocap, a large-scale high-quality synthetic dataset built for the task of egocentric whole-body motion capture. The EgoWholeMocap dataset is organized into two sections. The first part, containing over 700k frames, is rendered with 14 different rigged renderpeople~\cite{renderpeople} models driven by 2367 Mixamo~\cite{mixamo} motion sequences. It is worth noting that the Mixamo~\cite{mixamo} motions used in this part mainly focus on body movements, with less emphasis on hand motions. The second part of our dataset focuses on more complex hand motions and contains 170k frames with the SMPL-X model. This data is constructed from 24 different shapes and textures, driven by 200 motion sequences selected from the GRAB dataset~\cite{taheri2020grab} and 62 motion sequences from the TCDHandMocap dataset~\cite{hoyet2012sleight}. 

% Recognizing the need for more complex hand motion sequences, we introduce the second part of the EgoWholeMocap dataset, which contains over 170k frames. The second part is constructed with the SMPL-X model~\cite{pavlakos2019expressive} \DL{I would summarize this all as something like ``The second part of our dataset focuses on more complex hand motions and contains 170k frames with SMPL-X model. This data is constructed from 24 different...''} with 24 different shapes and textures, driven by 200 motion sequences selected from the GRAB dataset~\cite{taheri2020grab} and 62 motion sequences from the TCDHandMocap dataset~\cite{hoyet2012sleight}. 

During the rendering process, we first attach a virtual fisheye camera to the forehead of human body models and render the images, semantic labels, and depth map with Blender~\cite{blender}. The EgoWholeMocap dataset offers a valuable resource for advancing research in egocentric whole-body motion capture. It is larger and more diverse than previous egocentric training datasets---see Sec.~\ref{supp:dataset_comparison} in the supplementary material for a detailed comparison. \DL{I suggest that we make the paragraph in the intro about the dataset L085-L097 more high level, without giving too much details about each dataset used, and place these two last sentences from here there, to emphasize that our dataset is a valuable contribution.}

\subsection{Single Image Based Egocentric Pose Estimation} \label{method:single_image_pose}

% In this section, we propose a single-frame whole-body pose estimation method including three components: FisheyeViT (Sec.~\ref{method:fisheyevit}), pixel-aligned 3D heatmap (Sec.~\ref{method:pixel_aligned_heatmap}), and hand pose estimator (Sec.~\ref{method:wholebodypose}).
% In this section, we propose a whole-body pose estimation method that takes a single egocentric image as the input \DL{In general, the beginning of the sections are a bit repetitive. Since an overview was given in the beginning of Sec. 3, we can start the subsections more direct to the point}. Our method consists of three key components: FisheyeViT (Sec.~\ref{method:fisheyevit}), pixel-aligned 3D heatmap (Sec.~\ref{method:pixel_aligned_heatmap}), and hand pose estimator (Sec.~\ref{method:wholebodypose}).

\subsubsection{FisheyeViT} \label{method:fisheyevit}

\JW{Compare with previous method works on Paranoma}

In this section, we introduce FisheyeViT, which is specially designed to alleviate the fisheye distortion issue.
% FisheyeViT is specially designed to alleviate the fisheye distortion issue. 
Instead of undistorting the entire fisheye image, which is impractical due to its wide field of view, we extract undistorted image patches from the fisheye image and then fit these patches as tokens into the transformer network~\cite{dosovitskiy2020image}.
%
The FisheyeViT can be split into 5 steps, the first 4 of which are illustrated in Fig.~\ref{fig:fisheye_vit_inline}.
% Please refer to Fig.~\ref{fig:fisheye_vit_inline} for a detailed illustration of.
% For a detailed illustration, please refer to Fig.~\ref{fig:fisheye_vit_inline} and Sec.\ref{supp:fisheye_vit} in the supplementary materials. 
% Please also refer to Sec.~\ref{supp:fisheye_vit} and Fig.~\ref{fig:fisheye_vit} in the supplementary materials for the detailed illustration of FisheyeViT.

Step 1, given an input image $\mathbf{I}$ with size $H\times W$, we first evenly sample $N\times N$ patch center points: $\{\mathbf{C}_{ij} = (u_i, v_j) = \left(\frac{H}{N}(i + \frac{1}{2}), \frac{W}{N}(j + \frac{1}{2})\right) | i,j \in 0, 1, 2, ..., N-1\}$, where $i, j$ are the index of the point in row and in column. Then, the patch center points $\mathbf{C}_{ij}$ are projected into a unit sphere surface with the fisheye reprojection function: 
$\mathbf{P}^c_{ij} = (x^c_{ij}, y^c_{ij}, z^c_{ij}) = \mathcal{P}^{-1}(u_i, v_j, 1)$. The fisheye camera model is explained in Sec.~\ref{supp:fisheye_model} of supplementary materials. Given point $\mathbf{P}^c_{ij}$ on a unit sphere, the tangent plane $\mathbf{T}_{ij}$ that passes through the point is defined by the normal vector $\mathbf{v}^c_{ij} = (x^c_{ij}, y^c_{ij}, z^c_{ij})$. Next, we sample grid points in the plane and project them back to the fisheye image.

Step 2, in order to decide the scale and orientation of the grid points in the tangent plane, we select a 2D point in the fisheye image space which is $d$ pixels right to the patch center point: $\mathbf{U}_{ij} = (u_i + d, v_j)$, then this point is projected to the unit sphere surface with the fisheye reprojection function: $\mathbf{P}^u_{ij} = (x^u_{ij}, y^u_{ij}, z^u_{ij}) = \mathcal{P}^{-1}(u_i + d, v_j, 1)$. We next calculate the intersecting point $\mathbf{P}^x_{ij}$ between vector $\mathbf{v}^u_{ij} = (x^u_{ij}, y^u_{ij}, z^u_{ij})$ that is passing the original point $(0, 0, 0)$ and the tangent plane $\mathbf{T}_{ij}$: 
\begin{equation}
    \mathbf{P}^x_{ij} = \frac{\mathbf{P}^c_{ij} \cdot \mathbf{v}^c_{ij} }{\mathbf{v}^u_{ij} \cdot \mathbf{v}^c_{ij} } \mathbf{v}^u_{ij}
\end{equation}

\begin{figure}
\centering
\includegraphics[width=0.96\linewidth]{fig/fisheyevit/fisheyevit_inline_2_crop.pdf}
\caption{The detailed illustration of FisheyeViT (Sec.~\ref{method:fisheyevit}). \ZC{In step 3 fig, perhaps use different color for the arrows pointing to $\mathbf{V}^x_{ij})$ and $\mathbf{V}^v_{ij})$}
\vspace{-1em}
}
\label{fig:fisheye_vit_inline}
\end{figure}

Step 3, based on the center point $\mathbf{P}^c_{ij}$ and intersection point $\mathbf{P}^x_{ij}$ on the tangent plane $\mathbf{T}_{ij}$, we build a coordinate system with $x$ vector: $\mathbf{v}^x_{ij} = \text{Norm}(\mathbf{P}^x_{ij} - \mathbf{P}^c_{ij})$, $z$ vector: $\mathbf{v}^z_{ij} = \text{Norm}(\mathbf{v}^c_{ij})$ and $y$ vector: $\mathbf{v}^y_{ij} = \mathbf{v}^x_{ij} \times \mathbf{v}^z_{ij}$, where $\text{Norm}$ denotes the normalize operation. We grid-sample $M \times M$ points in a $l \times l$ square of the $x-y$ plane: 
\begin{equation}
    \{\mathbf{P}^{mn}_{ij} = \mathbf{P}^c_{ij} + (l\frac{m}{M} \mathbf{v}^x_{ij}, l\frac{n}{M} \mathbf{v}^y_{ij})\}
\end{equation}
where $m, n \in -\frac{1}{2}(M-1), ..., -\frac{3}{2}, -\frac{1}{2}, \frac{1}{2}, \frac{3}{2}, ... \frac{1}{2}(M-1)$. 

Step 4, the points $\mathbf{P}^{mn}_{ij}$ are projected back to the fisheye image with the fisheye projection function: $\mathbf{C}^{mn}_{ij} = \mathcal{P}(\mathbf{P}^{mn}_{ij})$. We use the bilinear sampling to sample the colors at points $\mathbf{C}^{mn}_{ij}$ of the input image $\mathbf{I}$ and reshape the sampled colors in $M \times M$ matrix, finally obtain the undistorted image patch $\mathbf{I}^{\text{undis}}_{ij}$. Please also refer to the supplementary video for the illustration of what the distorted image patches look like and how they move on the fisheye image.

Step 5, the image patches $\{\mathbf{I}^{\text{undis}}_{ij}\}$ are sent to a ViT transformer network~\cite{dosovitskiy2020image} and obtain the feature tokens $\{\mathbf{F}_{ij}\}$. The feature token is further reshaped in $i \times j$ matrix and obtain the image feature $\mathbf{F}$. In the FisheyeViT, we empirically set the numbers when the input image size $H=W=256$: $N=16; M=16; d=8; l=0.2m$.

It is worth noting that $\mathbf{C}^{mn}_{ij}$ is independent of the image $\mathbf{I}$. This means that, given a fixed fisheye camera model, we can precompute $\mathbf{C}^{mn}_{ij}$ for all combinations of $m, n$ and $i, j$ in advance. This significantly speeds up both the training and evaluation processes. Furthermore, the number and dimensions of image patches $\{\mathbf{I}^{\text{undis}}_{ij}\}$ match exactly with those in the traditional ViT network. This compatibility allows us to finetune existing ViT networks on our egocentric datasets.
Our sampling strategy ensures that each image patch $\mathbf{I}^{\text{undis}}_{ij}$ corresponds to the same FOV range in the fisheye camera. In our ablation study in Sec.~\ref{ablation_study}, we demonstrate that FisheyeViT significantly enhances the performance of the pose estimation network when applied to egocentric fisheye images.



\subsubsection{Pixel-Aligned 3D Heatmap} \label{method:pixel_aligned_heatmap}

After collecting image features with FisheyeViT, we utilize a 3D heatmap-based network to estimate the positions of 3D human body joints. The existing 3D heatmap approach~\cite{sun2018integral} is suitable for weak-perspective cameras but not for fisheye cameras. Therefore, we introduce a novel pose regressor that relies on the pixel-aligned 3D heatmap, tailored to address the needs of fisheye cameras. Given a feature map $\mathbf{F} \in \mathbb{R}^{C, H, W}$, where $C$ is the channel number, $H$ is the feature map height and $W$ is the feature map width, we firstly use a 1D convolution network to convert the feature map $\mathbf{F}$ into shape $(D \times J, H, W)$, and further reshape it to pixel-aligned 3D heatmap $\mathbf{H}\in \mathbb{R}^{J, D, H, W}$, where $J$ is the joint number and $D$ is the 3D heatmap depth. The illustration of $\mathbf{H}$ is shown in Fig.~\ref{fig:framework}. Next, we obtain the max-value positions $\mathbf{\tilde{J}}_b=\{(u_i, v_i, d_i) \mid i\in 0, 1, 2,..., J\}$ from $\mathbf{H}$ by the differentiable soft-argmax operation~\cite{sun2018integral}. Here, we note that $u_i$ and $v_i$ correspond to the uv-coordinate of the 3D body joint projected in the fisheye image space, and $d_i$ denotes the distance of the joint to the fisheye camera. Finally, the 3D body joints $\mathbf{\hat{J}}_b=\{(x_i, y_i, z_i) \mid i\in 0, 1, 2,..., J\}$ are recovered with the fisheye reprojection function: $(x_i, y_i, z_i) = \mathcal{P}^{-1}(u_i, v_i, d_i)$. The predicted body pose $\mathbf{\hat{J}}_b$ is finally compared with the ground truth body pose $\mathbf{J}_{b}$ from the EgoWholeMocap dataset with the MSE loss.

Our proposed pixel-aligned heatmap representation solves problems in all three types of previous egocentric joint regressors. 
First, Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} employs separate networks to predict 2D joint positions and joint distances and then calculates 3D joint positions using a fisheye reprojection function. However, this method can yield unrealistic joint estimations because small errors in 2D joints can result in large errors in 3D joints due to the projection effect. 
Second, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} and EgoHMR~\cite{liu2023egohmr} directly regress the 3D joint positions. However, this method is agnostic to the fisheye camera parameters, making it suitable only for a specific camera configuration (\eg, camera distortion parameters, focal length, head-mounted position, \etc). 
Third, SceneEgo~\cite{wang2023scene} projects 2D features into 3D voxel space with the fisheye reprojection function and uses a V2V network to regress 3D joints. However, this method suffers from low training and inference speed and large memory consumption, mainly because of the V2V network. In contrast to the above methods, our pixel-aligned 3D heatmap stands out for its simplicity and speed. It directly estimates 3D joints while also incorporating an explicitly parametrized fisheye camera model. This approach provides a more versatile and efficient solution to tackle the challenges in egocentric pose estimation. \ZC{we may need to discuss another main advantage of 3D heatmap repsentation -- its ability to perseve the uncertainty or confidence of the estimated joints, this uncertainty could be used in the diffusion refinement stage.} Detailed comparison with other pose prediction heads is shown in Table~\ref{table:ablation_study}.

\subsubsection{Egocentric Hand Pose Estimation} \label{method:wholebodypose}

In this section, we first train a network to detect hand pose locations and then train a 3D hand pose estimation network to regress 3D hand poses. Then, we describe how to integrate the estimated hand and body poses.

\noindent\textbf{Hand Detection}
Given an input image $\mathbf{I}$, we finetune the ViTPose~\cite{xu2022vitpose} network to regress the 2D hand poses of left hand $\mathbf{J}^{2d}_{lh}$ and right hand $\mathbf{J}^{2d}_{rh}$. From the 2D hand poses, we obtain the center point of left hand $\mathbf{C}_{lh}$ and right hand $\mathbf{C}_{rh}$, along with the bounding box sizes, $d_{lh}$ and $d_{rh}$ for the 2D hand poses. We use our approach described in Sec.~\ref{method:fisheyevit} to compute undistorted image patches of left $\mathbf{I}_{lh}$ and right hands $\mathbf{I}_{rh}$.

\noindent\textbf{Hand Pose Estimation}
Given the cropped image $\mathbf{I}_{lh}$ or $\mathbf{I}_{rh}$, we regress the 3D hand poses $\mathbf{\hat{J}}^{loc}_{lh}$ and $\mathbf{\hat{J}}^{loc}_{rh}$ with the Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} network, which is fine-tuned on our EgoFullBody dataset.

\noindent\textbf{Integration of body and hand poses}
It is not straightforward to integrate the hand poses with the body pose in the egocentric camera view primarily due to the fisheye camera's perspective effects. We can consider the left hand as an example. Following step 3 in Sec.~\ref{method:fisheyevit}, we establish a local coordinate system on the tangent plane of the left-hand image with XYZ axes as follows: $x: \mathbf{v}^x_{lh}$; $y: \mathbf{v}^y_{lh}$; $z: \mathbf{v}^z_{lh}$. We define a rotation matrix, denoted as $\mathbf{R}$, that represents the transformation between the root coordinate system and the local coordinate system on the tangent plane. The estimated hand pose is first rotated with the rotation matrix $\mathbf{\hat{J}}_{lh} = \mathbf{R}\mathbf{\hat{J}}^{loc}_{lh}$ and then translated to align the wrist location of the human body. This same process is also applied to the right hand to get the right hand pose $\mathbf{\hat{J}}_{rh}$. The whole-body joints $\mathbf{\hat{J}}$ are obtained by combining $\mathbf{\hat{J}}_{b}$,  $\mathbf{\hat{J}}_{lh}$, and $\mathbf{\hat{J}}_{rh}$. The uncertainty of whole-body joints $\mathbf{\hat{U}}$ is also obtained by finding the maximal value of the 3D heatmap in pose estimation modules.

\subsection{Diffusion-Based Motion Refinement} \label{method:diffusion}

We notice that the single-frame estimations in Sec.~\ref{method:single_image_pose} suffer from inaccuracies and temporal instabilities. In this section, we propose a diffusion-based motion refinement method to tackle this problem. We first learn the whole-body motion prior with the motion diffusion model in Sec.~\ref{method:wholebody_motion_diffusion} and then introduce an uncertainty-aware zero-shot motion refinement method in Sec.~\ref{method:uncertainty_aware}.

\subsubsection{Whole-Body Motion Diffusion Model} \label{method:wholebody_motion_diffusion}

% We introduce our whole-body motion encoding, represented as $\mathbf{x}$, which relies on the sequence of whole-body joints. Each whole-body joint $\mathbf{J}$ in the sequence is adjusted to its original position and aligned to face forward. Hand joints and body joints are separated and individually normalized. The root orientation and root velocity are combined with the normalized hand and body joints. This combined information is stacked frame by frame, resulting in the whole-body motion encoding $\mathbf{x}$.

We follow the DDPM~\cite{ho2020denoising} as our diffusion approach to capture the whole-body motion prior $q(\mathbf{x})$. DDPM learns a distribution of whole-body motion $\mathbf{x}$ through a forward diffusion process and an inverse denoising process. 
The forward diffusion process is a Markov process of adding Gaussian noise over $t \in \{0, 1, ..., T-1\}$ steps:
\begin{equation}
    q(\mathbf{x}_t|\mathbf{x}_{t-1}) = \mathcal{N}(\sqrt{\alpha_t}\mathbf{x}_{t-1}, (1 - \alpha_t)I)
\end{equation}
where $\mathbf{x}_t$ denotes the whole-body motion sequence at step $t$, the variance $(1-\alpha_t) \in (0, 1]$ denotes a constant hyperparameter increases with $t$. 

The inverse process uses a denoising network $D(\cdot)$ to remove the added Gaussian noise at each time step $t$. Here we use the transformer-based framework in EDGE~\cite{tseng2023edge} as the motion-denoising network $D(\cdot)$. We follow Ramesh~\etal's work~\cite{ramesh2022hierarchical} to make the network predict the original signal itself, \ie $\mathbf{\hat{x}}_0 = D(\mathbf{x}_t, t)$ and train it with the simple objective~\cite{ho2020denoising}:
\begin{equation}
    \mathcal{L}_{\text{simple}} = E_{\mathbf{x}_0 \sim q(\mathbf{x}_0), t \sim [1, T]}\left[ \vert\vert\mathbf{x}_0 - D(\mathbf{x}_t, t)\vert\vert^2_2 \right]
\end{equation}


\subsubsection{Uncertainty-Aware Motion Refinement} \label{method:uncertainty_aware}

Given the learned whole-body motion prior, we leverage the uncertainty value for each pose to guide the diffusion denoising process with the classifier-guided diffusion sampling~\cite{dhariwal2021diffusion}. Given an initial sequence of whole-body pose estimation $\mathbf{x}_e = \{\mathbf{\hat{J}}_i\}$ and the uncertainty value for each pose $\mathbf{u} = \{\mathbf{\hat{U}}_i\}$, where $i$ denotes the $i$th pose in the sequence, we keep the joints with low uncertainty but use the diffusion model to generate joints with high uncertainty conditioned upon the low-uncertainty joints. Specifically, in the $t$th sampling step of the diffusion process, the denoising network predicts $\mathbf{\hat{x}}_0 = D(\mathbf{x}_t, t)$, which is noised back to $\mathbf{x}_{t-1}$ by sampling from the Gaussian distribution:
% \begin{equation}
% \begin{split}
%     \mathbf{x}_{t-1} &\sim \mathcal{N}(\mathbf{\hat{x}}_0 + w(\mathbf{x}_e - \mathbf{\hat{x}}_0), \Sigma_t); \\
%     w &= (1 + \exp(-k(t-T\mathbf{u}_e)))^{-1}
% \end{split}
% \end{equation}
\begin{equation}
    \mathbf{x}_{t-1} \sim \mathcal{N}(\mathbf{\hat{x}}_0 + \mathbf{w}(\mathbf{x}_e - \mathbf{\hat{x}}_0), \Sigma_t)
\end{equation}
where $\Sigma_t$ is a scheduled Gaussian distribution in DDPM~\cite{ho2020denoising} and $\mathbf{w}$ controls the weight of a specific joint between the predicted motion $\mathbf{\hat{x}}_0$ and the estimated motion $\mathbf{x}_e$. Generally, we hope the $\mathbf{w} \rightarrow \overrightarrow{0}$ when $t \rightarrow 0$ such that the temporal stability is guaranteed through the generation of the denoising process, and $\mathbf{w} \rightarrow \overrightarrow{1}$ when $t \rightarrow T$ such that the denoising process is initialized by the estimated motion $\mathbf{x}_e$. We also hope that $w_{ij} = \mathbf{w}[i][j]$, which is the weight of $j$th joints in the $i$th pose, is smaller when the uncertainty value $u_{ij} = \mathbf{u}[i][j]$ of the $j$th joints in the $i$th pose is large. Based on this requirement, we design $\mathbf{w}$ as:
\begin{equation}
    \mathbf{w} = 1 / \left(1 + e^{-k(t-T\mathbf{u})}\right)
\end{equation}
where $T$ is the overall diffusion steps, $k$ is a hyperparameter which is empirically set to $0.1$.
% \ZC{perhaps need to add ablations of different $\mathbf{w}$ function choices in the supplement} 
From the experimental results in Sec.~\ref{experiments}, we demonstrate the effectiveness of uncertain-aware motion refinement and our uncertainty-guided diffusion sampling strategy.



==> sec/bak/3_method_bak2.tex <==
\section{Method} \label{method}
In this section, we propose a new method for predicting accurate egocentric whole-body poses from egocentric image sequences. An overview of our approach is shown in Fig.~\ref{fig:framework}. 
% We propose a single-frame whole-body pose estimation method including three components: the FisheyeViT (Sec.~\ref{method:fisheyevit}) the pixel-aligned 3D heatmap (Sec.~\ref{method:pixel_aligned_heatmap}) and the hand pose estimator (Sec.~\ref{method:wholebodypose}). Finally, we refine the combined human hand and body motion with the uncertainty-aware diffusion model (Sec.~\ref{method:diffusion}).
% \DL{A general comment is that we already mention a quite detailed overview of all the steps in the method back in the introduction; then we mention it here again in a more high level. I think that, if we already mention an overview in the intro L040-L097, we can skip it here;}



\subsection{Single Image Based Egocentric Pose Estimation} \label{method:single_image_pose}

\subsubsection{FisheyeViT} \label{method:fisheyevit}

In this section, we introduce FisheyeViT, which is specially designed to alleviate the fisheye distortion issue. Instead of undistorting the entire fisheye image, which is impractical due to its wide field of view, we extract undistorted image patches from the fisheye image and then fit these patches as tokens into the transformer network~\cite{dosovitskiy2020image}. 
% \JW{
To get the undistorted patches, we first warp the fisheye image to a unit semi-sphere, then get the patches with the gnomonic projection (see Figure~\ref{fig:framework}).
% }
The FisheyeViT can be split into five steps, the first four of which are illustrated in Fig.~\ref{fig:fisheye_vit_inline}.

\textbf{Step 1.} Given an input image $\mathbf{I}$ with size $H\times W$, we first evenly sample $N\times N$ patch center points: $\{\mathbf{C}_{ij} = (u_i, v_j) = \left(\frac{H}{N}(i + \frac{1}{2}), \frac{W}{N}(j + \frac{1}{2})\right) | i,j \in 0, 1, 2, ..., N-1\}$, where $i, j$ are the index of the point in row and in column. Then, the patch center points $\mathbf{C}_{ij}$ are projected onto a unit sphere surface with the fisheye reprojection function: 
$\mathbf{P}^c_{ij} = (x^c_{ij}, y^c_{ij}, z^c_{ij}) = \mathcal{P}^{-1}(u_i, v_j, 1)$. The fisheye camera model is shown in Sec.~\ref{supp:fisheye_model} of supplementary materials. Given a point $\mathbf{P}^c_{ij}$ on a unit sphere, the tangent plane $\mathbf{T}_{ij}$ that passes through the point is defined by the normal vector $\mathbf{v}^c_{ij} = (x^c_{ij}, y^c_{ij}, z^c_{ij})$. In the next steps, we implement the gnomonic projection by sampling grid points in the plane and projecting them back to the fisheye image.

\textbf{Step 2.} In this step, we decide the orientation of the grid points in the tangent plane. 
% \JW{
We aim to ensure that the grid points from different tangent planes $\mathbf{T}_{ij}$ have the same orientation when projected back onto the fisheye image. To achieve this,
% }
we select a 2D point in the fisheye image space which is $d$ pixels right to the patch center point: $\mathbf{U}_{ij} = (u_i + d, v_j)$, then this point is projected to the unit sphere surface with the fisheye reprojection function: $\mathbf{P}^u_{ij} = (x^u_{ij}, y^u_{ij}, z^u_{ij}) = \mathcal{P}^{-1}(u_i + d, v_j, 1)$. We next calculate the intersection point $\mathbf{P}^x_{ij}$ between vector $\mathbf{v}^u_{ij} = (x^u_{ij}, y^u_{ij}, z^u_{ij})$ that is passing the original point $(0, 0, 0)$ and the tangent plane $\mathbf{T}_{ij}$: 
\begin{equation}
    \mathbf{P}^x_{ij} = \frac{\mathbf{P}^c_{ij} \cdot \mathbf{v}^c_{ij} }{\mathbf{v}^u_{ij} \cdot \mathbf{v}^c_{ij} } \mathbf{v}^u_{ij}
\end{equation}

\begin{figure}
\centering
\includegraphics[width=0.96\linewidth]{fig/fisheyevit/fisheyevit_inline_color_crop.pdf}
\caption{The detailed illustration of FisheyeViT (Sec.~\ref{method:fisheyevit}).
\vspace{-1em}
}
\label{fig:fisheye_vit_inline}
\end{figure}

\textbf{Step 3.} Based on the center point $\mathbf{P}^c_{ij}$ and intersection point $\mathbf{P}^x_{ij}$ on the tangent plane $\mathbf{T}_{ij}$, we build a coordinate system with the $x$ axis: $\mathbf{v}^x_{ij} = \text{Norm}(\mathbf{P}^x_{ij} - \mathbf{P}^c_{ij})$, the $z$ axis: $\mathbf{v}^z_{ij} = \text{Norm}(\mathbf{v}^c_{ij})$ and the $y$ axis: $\mathbf{v}^y_{ij} = \mathbf{v}^z_{ij} \times \mathbf{v}^x_{ij}$, where $\text{Norm}$ denotes the normalize operation. We grid-sample $M \times M$ points in a $l \times l$ square of the $x\text{-}y$ plane: 
\begin{equation}
    \{\mathbf{P}^{mn}_{ij} = \mathbf{P}^c_{ij} + (l\frac{m}{M} \mathbf{v}^x_{ij}, l\frac{n}{M} \mathbf{v}^y_{ij})\}
\end{equation}
where $m, n \in -\frac{1}{2}(M-1), ..., -\frac{3}{2}, -\frac{1}{2}, \frac{1}{2}, \frac{3}{2}, ... \frac{1}{2}(M-1)$. 

\textbf{Step 4.} The points $\mathbf{P}^{mn}_{ij}$ are projected back to the fisheye image with the fisheye projection function: $\mathbf{C}^{mn}_{ij} = \mathcal{P}(\mathbf{P}^{mn}_{ij})$. We then apply the bilinear sampling to obtain the colors at points $\mathbf{C}^{mn}_{ij}$ of the input image $\mathbf{I}$ and reshape the sampled colors in $M \times M$ matrix, and finally obtain the undistorted image patch $\mathbf{I}^{\text{undis}}_{ij}$. 
Please also see the supplementary video for a visual demonstration of undistorted image patches and their movement on the fisheye image.
% Please also see the supplementary video for the illustration of what the undistorted image patches look like and how they move on the fisheye image.

\textbf{Step 5.} The image patches $\{\mathbf{I}^{\text{undis}}_{ij}\}$ are sent to a ViT transformer network~\cite{dosovitskiy2020image} to obtain the feature tokens $\{\mathbf{F}_{ij}\}$. The feature token is further reshaped in $i \times j$ matrix and obtain the image feature $\mathbf{F}$. In the FisheyeViT, we empirically set the numbers when the input image size $H=W=256$: $N=16; M=16; d=8; l=0.2m$.

Note that $\mathbf{C}^{mn}_{ij}$ is independent of the image $\mathbf{I}$. This means that, given a fixed fisheye camera model, we can precompute $\mathbf{C}^{mn}_{ij}$ for all combinations of $m, n$ and $i, j$ in advance. This significantly speeds up both the training and evaluation processes. Furthermore, the number and dimensions of image patches $\{\mathbf{I}^{\text{undis}}_{ij}\}$ match exactly with those in the traditional ViT network. This compatibility allows us to finetune existing ViT networks on our egocentric datasets.
Our sampling strategy ensures that each image patch $\mathbf{I}^{\text{undis}}_{ij}$ corresponds to the same FOV range in the fisheye camera. In our ablation study in Sec.~\ref{ablation_study}, we show that FisheyeViT enhances the performance of the pose estimation network when applied to egocentric fisheye images.



\subsubsection{Pixel-Aligned 3D Heatmap} \label{method:pixel_aligned_heatmap}

After collecting image features with FisheyeViT, we utilize a 3D heatmap-based network to estimate the positions of 3D human body joints. The existing 3D heatmap approach~\cite{sun2018integral} is designed for weak-perspective cameras but not for fisheye cameras. Therefore, we introduce a novel pose regressor that relies on the pixel-aligned 3D heatmap, tailored to address the needs of fisheye cameras. \ZC{same issue as intro, I think both heatmaps are pixel-aligned} Given a feature map $\mathbf{F} \in \mathbb{R}^{C \times N \times N}$, where $C$ is the channel number, $N$ is feature map height and width, we firstly use two deconvolutional layers to convert the feature map $\mathbf{F}$ into shape $(D_h \times J, H_h, W_h)$, and further reshape it to pixel-aligned 3D heatmap $\mathbf{H}\in \mathbb{R}^{J \times D_h \times H_h \times W_h}$, where $J$ is the joint number and $D_h$, $H_h$, $W_h$ is the 3D heatmap depth, height and width. The illustration of $\mathbf{H}$ is shown in Fig.~\ref{fig:framework}. Next, we obtain the max-value positions $\mathbf{\tilde{J}}_b=\{(u_i, v_i, d_i) \mid i\in 0, 1, 2,..., J\}$ from $\mathbf{H}$ by the differentiable soft-argmax operation~\cite{sun2018integral}. Here, we note that $u_i$ and $v_i$ correspond to the uv-coordinate of the 3D body joint projected in the fisheye image space, and $d_i$ denotes the distance of the joint to the fisheye camera. Finally, the 3D body joints $\mathbf{\hat{J}}_b=\{(x_i, y_i, z_i) \mid i\in 0, 1, 2,..., J\}$ are recovered with the fisheye reprojection function: $(x_i, y_i, z_i) = \mathcal{P}^{-1}(u_i, v_i, d_i)$. The predicted body pose $\mathbf{\hat{J}}_b$ is finally compared with the ground truth body pose $\mathbf{J}_{b}$ with the MSE loss. \JW{We prove that the heatmap can also be used under the fisheye setup. To ensure the pixel-align feature, we apply the transformation on the extracted pose.}

% After collecting image features with FisheyeViT, we utilize a 3D heatmap-based network to estimate the positions of 3D human body joints. The existing 3D heatmap approach~\cite{sun2018integral} is suitable for weak-perspective cameras but not for fisheye cameras. Therefore, we introduce a novel pose regressor that relies on the pixel-aligned 3D heatmap, tailored to address the needs of fisheye cameras. Given a feature map $\mathbf{F} \in \mathbb{R}^{C \times H \times W}$, where $C$ is the channel number, $H$ is the feature map height and $W$ is the feature map width, we firstly use a 1D convolution network to convert the feature map $\mathbf{F}$ into shape $(D \times J, H, W)$, and further reshape it to pixel-aligned 3D heatmap $\mathbf{H}\in \mathbb{R}^{J \times D \times H \times W}$, where $J$ is the joint number and $D$ is the 3D heatmap depth. The illustration of $\mathbf{H}$ is shown in Fig.~\ref{fig:framework}. Next, we obtain the max-value positions $\mathbf{\tilde{J}}_b=\{(u_i, v_i, d_i) \mid i\in 0, 1, 2,..., J\}$ from $\mathbf{H}$ by the differentiable soft-argmax operation~\cite{sun2018integral}. Here, we note that $u_i$ and $v_i$ correspond to the uv-coordinate of the 3D body joint projected in the fisheye image space, and $d_i$ denotes the distance of the joint to the fisheye camera. Finally, the 3D body joints $\mathbf{\hat{J}}_b=\{(x_i, y_i, z_i) \mid i\in 0, 1, 2,..., J\}$ are recovered with the fisheye reprojection function: $(x_i, y_i, z_i) = \mathcal{P}^{-1}(u_i, v_i, d_i)$. The predicted body pose $\mathbf{\hat{J}}_b$ is finally compared with the ground truth body pose $\mathbf{J}_{b}$ with the MSE loss.

\JW{make it shorter}
Our proposed pixel-aligned heatmap representation solves problems in all three types of previous egocentric joint regressors. 
First, Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} employs separate networks to predict 2D joint positions and joint distances and then calculates 3D joint positions using a fisheye reprojection function. However, this method can yield unrealistic joint estimations because small errors in 2D joints can result in large errors in 3D joints due to the projection effect. 
Second, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} and EgoHMR~\cite{liu2023egohmr} directly regress the 3D joint positions. However, this method is agnostic to the fisheye camera parameters, making it suitable only for a specific camera configuration (\eg, camera distortion parameters, focal length, head-mounted position, \etc). 
Third, SceneEgo~\cite{wang2023scene} projects 2D features into 3D voxel space with the fisheye reprojection function and uses a V2V network to regress 3D joints. However, this method suffers from low training and inference speed and large memory consumption, mainly because of the V2V network. In contrast to the above methods, our pixel-aligned 3D heatmap stands out for its simplicity and speed. It directly estimates 3D joints while also incorporating an explicitly parametrized fisheye camera model. This approach provides a more versatile and efficient solution to tackle the challenges in egocentric pose estimation. Moreover, it can preserve the uncertainty of the estimated joints, which will be used in our uncertainty-aware motion refinement method (Sec.~\ref{method:uncertainty_aware}). Detailed comparison with other pose prediction heads is shown in Table~\ref{table:ablation_study}.

\subsubsection{Egocentric Hand Pose Estimation} \label{method:wholebodypose}

In this section, we first train a network to detect hand pose locations and then train a 3D hand pose estimation network to regress 3D hand poses. Then, we describe how to integrate the estimated hand and body poses.

\noindent\textbf{Hand Detection.}
Given an input image $\mathbf{I}$, we finetune the ViTPose~\cite{xu2022vitpose} network to regress the 2D hand poses of left hand $\mathbf{J}^{2d}_{lh}$ and right hand $\mathbf{J}^{2d}_{rh}$. From the 2D hand poses, we obtain the center point of left hand $\mathbf{C}_{lh}$ and right hand $\mathbf{C}_{rh}$, along with the bounding box sizes, $d_{lh}$ and $d_{rh}$ for the 2D hand poses. We use our approach described in Sec.~\ref{method:fisheyevit} to compute undistorted image patches of left $\mathbf{I}_{lh}$ and right hands $\mathbf{I}_{rh}$.

\noindent\textbf{Hand Pose Estimation.}
Given the cropped image $\mathbf{I}_{lh}$ or $\mathbf{I}_{rh}$, we regress the 3D hand poses $\mathbf{\hat{J}}^{loc}_{lh}$ and $\mathbf{\hat{J}}^{loc}_{rh}$ with the Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} network, which is fine-tuned on our EgoFullBody dataset.

\noindent\textbf{Integration of Body and Hand Poses.}
It is not straightforward to integrate the hand poses with the body pose in the egocentric camera view primarily due to the fisheye camera's perspective effects. Take the left hand as an example. Following Step 3 in Sec.~\ref{method:fisheyevit}, we establish a local coordinate system on the tangent plane of the left-hand image with XYZ axes as follows: $x: \mathbf{v}^x_{lh}$; $y: \mathbf{v}^y_{lh}$; $z: \mathbf{v}^z_{lh}$. We define a rotation matrix, denoted as $\mathbf{R}$, that represents the transformation between the root coordinate system and the local coordinate system on the tangent plane. The estimated hand pose is first rotated with the rotation matrix $\mathbf{\hat{J}}_{lh} = \mathbf{R}\mathbf{\hat{J}}^{loc}_{lh}$ and then translated to align the wrist location of the human body. This same process is also applied to the right hand to get the right hand pose $\mathbf{\hat{J}}_{rh}$. The whole-body joints $\mathbf{\hat{J}}$ are obtained by combining $\mathbf{\hat{J}}_{b}$,  $\mathbf{\hat{J}}_{lh}$, and $\mathbf{\hat{J}}_{rh}$. The uncertainty of whole-body joints $\mathbf{\hat{U}}$ is also obtained from the maximal value of the 3D heatmap in pose estimation modules.

\subsection{Diffusion-Based Motion Refinement} \label{method:diffusion}

We notice that the single-frame estimations in Sec.~\ref{method:single_image_pose} suffer from inaccuracies and temporal instabilities. In this section, we propose a diffusion-based motion refinement method to tackle this problem. We first learn the whole-body motion prior with the motion diffusion model in Sec.~\ref{method:wholebody_motion_diffusion} and then introduce an uncertainty-aware zero-shot motion refinement method in Sec.~\ref{method:uncertainty_aware}.

\subsubsection{Whole-Body Motion Diffusion Model} \label{method:wholebody_motion_diffusion}

% We introduce our whole-body motion encoding, represented as $\mathbf{x}$, which relies on the sequence of whole-body joints. Each whole-body joint $\mathbf{J}$ in the sequence is adjusted to its original position and aligned to face forward. Hand joints and body joints are separated and individually normalized. The root orientation and root velocity are combined with the normalized hand and body joints. This combined information is stacked frame by frame, resulting in the whole-body motion encoding $\mathbf{x}$.

We follow DDPM~\cite{ho2020denoising} as our diffusion approach to capture the whole-body motion prior $q(\mathbf{x})$. DDPM learns a distribution of whole-body motion $\mathbf{x}$ through a forward diffusion process and an inverse denoising process. 
The forward diffusion process is a Markov process of adding Gaussian noise over $t \in \{0, 1, ..., T-1\}$ steps:
\begin{equation}
    q(\mathbf{x}_t|\mathbf{x}_{t-1}) = \mathcal{N}(\sqrt{\alpha_t}\mathbf{x}_{t-1}, (1 - \alpha_t)I)
\end{equation}
where $\mathbf{x}_t$ denotes the whole-body motion sequence at step $t$, the variance $(1-\alpha_t) \in (0, 1]$ denotes a constant hyperparameter increases with $t$. 

The inverse process uses a denoising network $D(\cdot)$ to remove the added Gaussian noise at each time step $t$. Here we use the transformer-based framework in EDGE~\cite{tseng2023edge} as the motion-denoising network $D(\cdot)$. We follow Ramesh~\etal's work~\cite{ramesh2022hierarchical} to make the network predict the original signal itself, \ie $\mathbf{\hat{x}}_0 = D(\mathbf{x}_t, t)$ and train it with the simple objective~\cite{ho2020denoising}:
\begin{equation}
    \mathcal{L}_{\text{simple}} = E_{\mathbf{x}_0 \sim q(\mathbf{x}_0), t \sim [1, T]}\left[ \vert\vert\mathbf{x}_0 - D(\mathbf{x}_t, t)\vert\vert^2_2 \right]
\end{equation}


\subsubsection{Uncertainty-Aware Motion Refinement} \label{method:uncertainty_aware}

Given the learned whole-body motion prior, we leverage the uncertainty value for each pose to guide the diffusion denoising process with the classifier-guided diffusion sampling~\cite{dhariwal2021diffusion}. Given an initial sequence of whole-body pose estimation $\mathbf{x}_e = \{\mathbf{\hat{J}}_i\}$ and the uncertainty value for each pose $\mathbf{u} = \{\mathbf{\hat{U}}_i\}$, where $i$ denotes the $i$th pose in the sequence, we keep the joints with low uncertainty but use the diffusion model to generate joints with high uncertainty conditioned on the low-uncertainty joints. Specifically, in the $t$th sampling step of the diffusion process, the denoising network predicts $\mathbf{\hat{x}}_0 = D(\mathbf{x}_t, t)$, which is noised back to $\mathbf{x}_{t-1}$ by sampling from the Gaussian distribution:
% \begin{equation}
% \begin{split}
%     \mathbf{x}_{t-1} &\sim \mathcal{N}(\mathbf{\hat{x}}_0 + w(\mathbf{x}_e - \mathbf{\hat{x}}_0), \Sigma_t); \\
%     w &= (1 + \exp(-k(t-T\mathbf{u}_e)))^{-1}
% \end{split}
% \end{equation}
\begin{equation}
    \mathbf{x}_{t-1} \sim \mathcal{N}(\mathbf{\hat{x}}_0 + \mathbf{w}(\mathbf{x}_e - \mathbf{\hat{x}}_0), \Sigma_t)
\end{equation}
where $\Sigma_t$ is a scheduled Gaussian distribution in DDPM~\cite{ho2020denoising} and $\mathbf{w}$ controls the weight of a specific joint between the predicted motion $\mathbf{\hat{x}}_0$ and the estimated motion $\mathbf{x}_e$. Generally, we expect $\mathbf{w} \rightarrow \overrightarrow{0}$ when $t \rightarrow 0$ such that the temporal stability is guaranteed through the generation of the denoising process, and $\mathbf{w} \rightarrow \overrightarrow{1}$ when $t \rightarrow T$ such that the denoising process is initialized by the estimated motion $\mathbf{x}_e$. We also expect that $w_{ij} = \mathbf{w}[i][j]$, which is the weight of $j$th joints in the $i$th pose, is smaller when the uncertainty value $u_{ij} = \mathbf{u}[i][j]$ of the $j$th joints in the $i$th pose is large. Based on this requirement, we design $\mathbf{w}$ as:
\begin{equation}
    \mathbf{w} = 1 / \left(1 + e^{-k(t-T\mathbf{u})}\right)
\end{equation}
where $T$ is the overall diffusion steps, $k$ is a hyperparameter which is empirically set to $0.1$.
% \ZC{perhaps need to add ablations of different $\mathbf{w}$ function choices in the supplement} 
From the experimental results in Sec.~\ref{experiments}, we demonstrate the effectiveness of uncertain-aware motion refinement and our uncertainty-guided diffusion sampling strategy.


\section{EgoWholeMocap Dataset} \label{method:synthetic_dataset}

In this section, we introduce EgoWholeMocap, a large-scale high-quality synthetic dataset built for the task of egocentric whole-body motion capture. The EgoWholeMocap dataset is organized into two sections. The first part, containing over 700k frames, is rendered with 14 different rigged Renderpeople~\cite{renderpeople} models driven by 2367 Mixamo~\cite{mixamo} motion sequences. Note that the Mixamo~\cite{mixamo} motions used in this part mainly focus on body movements, lacking diversity in hand motions. The second part of our dataset focuses on more complex hand motions and contains 170k frames with the SMPL-X model. This data is constructed from 24 different shapes and textures, driven by 200 motion sequences selected from the GRAB dataset~\cite{taheri2020grab} and 62 motion sequences from the TCDHandMocap dataset~\cite{hoyet2012sleight}. 

During the rendering process, we first attach a virtual fisheye camera to the forehead of human body models and render the images, semantic labels, and depth map with Blender~\cite{blender}. 
% The EgoWholeMocap dataset offers a valuable resource for advancing research in egocentric whole-body motion capture. 
Our dataset is larger and more diverse than previous egocentric training datasets--see Sec.~\ref{supp:dataset_comparison} in the supplementary material for a detailed comparison. 
% \DL{I suggest that we make the paragraph in the intro about the dataset L085-L097 more high level, without giving too much details about each dataset used, and place these two last sentences from here there, to emphasize that our dataset is a valuable contribution.}

==> sec/bak/3_method_before_thabo.tex <==
\section{Method} \label{method}
In this section, we propose a new method for predicting accurate egocentric whole-body poses from egocentric image sequences. An overview of our approach is shown in Fig.~\ref{fig:framework}. 
% We propose a single-frame whole-body pose estimation method including three components: the FisheyeViT (Sec.~\ref{method:fisheyevit}) the pixel-aligned 3D heatmap (Sec.~\ref{method:pixel_aligned_heatmap}) and the hand pose estimator (Sec.~\ref{method:wholebodypose}). Finally, we refine the combined human hand and body motion with the uncertainty-aware diffusion model (Sec.~\ref{method:diffusion}).
% \DL{A general comment is that we already mention a quite detailed overview of all the steps in the method back in the introduction; then we mention it here again in a more high level. I think that, if we already mention an overview in the intro L040-L097, we can skip it here;}



\subsection{Single Image Based Egocentric Pose Estimation} \label{method:single_image_pose}

\subsubsection{FisheyeViT} \label{method:fisheyevit}

In this section, we introduce FisheyeViT, which is specially designed to alleviate the fisheye distortion issue. Instead of undistorting the entire fisheye image, we extract undistorted image patches from the fisheye image and then fit these patches as tokens into the transformer network~\cite{dosovitskiy2020image}. 
% \JW{
To get the undistorted patches, we first warp the fisheye image to a unit semi-sphere, then get the patches with the gnomonic projection (see \cref{fig:framework}).
% }
The FisheyeViT can be split into five steps, the first four of which are illustrated in Fig.~\ref{fig:fisheye_vit_inline}.

\textbf{Step 1.} Given an input image $\mathbf{I}$ with size $H\times W$, we first evenly sample $N\times N$ patch center points: $\{\mathbf{C}_{ij} = (u_i, v_j) = \left(\frac{H}{N}(i + \frac{1}{2}), \frac{W}{N}(j + \frac{1}{2})\right) | i,j \in 0, ..., N-1\}$. Then, the patch center points $\mathbf{C}_{ij}$ are projected onto a unit sphere with the fisheye reprojection function: 
$\mathbf{P}^c_{ij} = (x^c_{ij}, y^c_{ij}, z^c_{ij}) = \mathcal{P}^{-1}(u_i, v_j, 1)$. The fisheye camera model is shown in Sec.~\ref{supp:fisheye_model} of supplementary materials. Given a point $\mathbf{P}^c_{ij}$ on a unit sphere, the tangent plane $\mathbf{T}_{ij}$ that passes through the point is defined by the normal vector $\mathbf{v}^c_{ij} = (x^c_{ij}, y^c_{ij}, z^c_{ij})$. In the next steps, we implement the gnomonic projection by sampling grid points in the plane and projecting them back to the fisheye image.

\textbf{Step 2.} In this step, we decide the orientation of the grid points in the tangent plane. 
% \JW{
We aim to ensure that the grid points from different tangent planes $\mathbf{T}_{ij}$ have the same orientation when projected back onto the fisheye image. To achieve this,
% }
we select a 2D point in the fisheye image space which is $d$ pixels right to the patch center point: $\mathbf{U}_{ij} = (u_i + d, v_j)$, then this point is projected to the unit sphere surface with the fisheye reprojection function: $\mathbf{P}^u_{ij} = (x^u_{ij}, y^u_{ij}, z^u_{ij}) = \mathcal{P}^{-1}(u_i + d, v_j, 1)$. We next calculate the intersection point $\mathbf{P}^x_{ij}$ between vector $\mathbf{v}^u_{ij} = (x^u_{ij}, y^u_{ij}, z^u_{ij})$ that is passing the original point $(0, 0, 0)$ and the tangent plane $\mathbf{T}_{ij}$: 
\begin{equation}
    \mathbf{P}^x_{ij} = \frac{\mathbf{P}^c_{ij} \cdot \mathbf{v}^c_{ij} }{\mathbf{v}^u_{ij} \cdot \mathbf{v}^c_{ij} } \mathbf{v}^u_{ij}
\end{equation}

\begin{figure}
\centering
\includegraphics[width=0.96\linewidth]{fig/fisheyevit/fisheyevit_inline_color_crop.pdf}
\caption{The detailed illustration of FisheyeViT (Sec.~\ref{method:fisheyevit}).
\vspace{-1em}
}
\label{fig:fisheye_vit_inline}
\end{figure}

\textbf{Step 3.} Based on the center point $\mathbf{P}^c_{ij}$ and intersection point $\mathbf{P}^x_{ij}$ on the tangent plane $\mathbf{T}_{ij}$, we build a coordinate system with the $x$ axis: $\mathbf{v}^x_{ij} = \text{Norm}(\mathbf{P}^x_{ij} - \mathbf{P}^c_{ij})$, the $z$ axis: $\mathbf{v}^z_{ij} = \text{Norm}(\mathbf{v}^c_{ij})$ and the $y$ axis: $\mathbf{v}^y_{ij} = \mathbf{v}^z_{ij} \times \mathbf{v}^x_{ij}$, where $\text{Norm}$ denotes the normalize operation. We grid-sample $M \times M$ points in a $l \times l$ square of the $x\text{-}y$ plane: 
\begin{equation}
    \{\mathbf{P}^{mn}_{ij} = \mathbf{P}^c_{ij} + (l\frac{m}{M} \mathbf{v}^x_{ij}, l\frac{n}{M} \mathbf{v}^y_{ij})\}
\end{equation}
where $m, n \in -\frac{1}{2}(M-1), ..., -\frac{3}{2}, -\frac{1}{2}, \frac{1}{2}, \frac{3}{2}, ... \frac{1}{2}(M-1)$. 

\textbf{Step 4.} The points $\mathbf{P}^{mn}_{ij}$ are projected back to the fisheye image with the fisheye projection function: $\mathbf{C}^{mn}_{ij} = \mathcal{P}(\mathbf{P}^{mn}_{ij})$. We then apply the bilinear sampling to obtain the colors at points $\mathbf{C}^{mn}_{ij}$ of the input image $\mathbf{I}$ and reshape the sampled colors in $M \times M$ matrix, and finally obtain the undistorted image patch $\mathbf{I}^{\text{undis}}_{ij}$. 
Please also see the supplementary video for a visual demonstration of undistorted image patches and their movement on the fisheye image.
% Please also see the supplementary video for the illustration of what the undistorted image patches look like and how they move on the fisheye image.

\textbf{Step 5.} The image patches $\{\mathbf{I}^{\text{undis}}_{ij}\}$ are sent to a ViT transformer network~\cite{dosovitskiy2020image} to obtain the feature tokens $\{\mathbf{F}_{ij}\}$. The feature token is further reshaped in $i \times j$ matrix and obtain the image feature $\mathbf{F}$. In the FisheyeViT, we empirically set the numbers when the input image size $H=W=256$: $N=16; M=16; d=8; l=0.2m$.

Note that $\mathbf{C}^{mn}_{ij}$ is independent of the image $\mathbf{I}$. This means that, given a fixed fisheye camera model, we can precompute $\mathbf{C}^{mn}_{ij}$ for all combinations of $m, n$ and $i, j$ in advance. This significantly speeds up both the training and evaluation processes. Furthermore, the number and dimensions of image patches $\{\mathbf{I}^{\text{undis}}_{ij}\}$ match exactly with those in the traditional ViT network. This compatibility allows us to finetune existing ViT networks on our egocentric datasets.
Our sampling strategy ensures that each image patch $\mathbf{I}^{\text{undis}}_{ij}$ corresponds to the same FOV range in the fisheye camera. In our ablation study in Sec.~\ref{ablation_study}, we show that FisheyeViT enhances the performance of the pose estimation network when applied to egocentric fisheye images.



\subsubsection{Pixel-Aligned 3D Heatmap} \label{method:pixel_aligned_heatmap}

After collecting image features with FisheyeViT, we utilize a 3D heatmap-based network to estimate the body poses. The existing 3D heatmap-based pose regressors~\cite{sun2018integral, Moon_2022_CVPRW_Hand4Whole} are designed for weak-perspective cameras but are not compatible with fisheye cameras. 
% \JW{
Directly applying these regressors will result in the misalignment between 3D heatmap features in 3D space and 2D image features in fisheye image space. Therefore, we introduce a novel pose regressor that relies on the pixel-aligned 3D heatmap, tailored to address the needs of fisheye cameras. The idea is to regress the 3D heatmap in $uvd$ space rather than traditional  $xyz$ space, where $uv$ corresponds to the fisheye image $uv$ space.
% }
Specifically, given a feature map $\mathbf{F} \in \mathbb{R}^{C \times N \times N}$, where $C$ is the channel number, $N$ is feature map height and width, we firstly use two deconvolutional layers to convert the feature map $\mathbf{F}$ into shape $(D_h \times J, H_h, W_h)$, and further reshape it to pixel-aligned 3D heatmap $\mathbf{H}\in \mathbb{R}^{J \times D_h \times H_h \times W_h}$, where $J$ is the joint number and $D_h$, $H_h$, $W_h$ is the 3D heatmap depth, height and width. The illustration of $\mathbf{H}$ is shown in Fig.~\ref{fig:framework}. Next, we obtain the max-value positions $\mathbf{\tilde{J}}_b=\{(u_i, v_i, d_i) \mid i\in 0, 1, 2,..., J\}$ from $\mathbf{H}$ by the differentiable soft-argmax operation~\cite{sun2018integral}. Here, we note that $u_i$ and $v_i$ correspond to the uv-coordinate of the 3D body joint projected in the fisheye image space, and $d_i$ denotes the distance of the joint to the fisheye camera. Finally, the 3D body joints $\mathbf{\hat{J}}_b=\{(x_i, y_i, z_i) \mid i\in 0, 1, 2,..., J\}$ are recovered with the fisheye reprojection function: $(x_i, y_i, z_i) = \mathcal{P}^{-1}(u_i, v_i, d_i)$. The predicted body pose $\mathbf{\hat{J}}_b$ is finally compared with the ground truth body pose $\mathbf{J}_{b}$ with the MSE loss. 
% \JW{
By firstly regressing 3D body poses in $uvd$ space and then reprojecting it, we ensure that the 3D heatmap is pixel-aligned with the end-to-end training.
% }

% After collecting image features with FisheyeViT, we utilize a 3D heatmap-based network to estimate the positions of 3D human body joints. The existing 3D heatmap approach~\cite{sun2018integral} is designed for weak-perspective cameras but not for fisheye cameras. Therefore, we introduce a novel pose regressor that relies on the pixel-aligned 3D heatmap, tailored to address the needs of fisheye cameras. \ZC{same issue as intro, I think both heatmaps are pixel-aligned} Given a feature map $\mathbf{F} \in \mathbb{R}^{C \times N \times N}$, where $C$ is the channel number, $N$ is feature map height and width, we firstly use two deconvolutional layers to convert the feature map $\mathbf{F}$ into shape $(D_h \times J, H_h, W_h)$, and further reshape it to pixel-aligned 3D heatmap $\mathbf{H}\in \mathbb{R}^{J \times D_h \times H_h \times W_h}$, where $J$ is the joint number and $D_h$, $H_h$, $W_h$ is the 3D heatmap depth, height and width. The illustration of $\mathbf{H}$ is shown in Fig.~\ref{fig:framework}. Next, we obtain the max-value positions $\mathbf{\tilde{J}}_b=\{(u_i, v_i, d_i) \mid i\in 0, 1, 2,..., J\}$ from $\mathbf{H}$ by the differentiable soft-argmax operation~\cite{sun2018integral}. Here, we note that $u_i$ and $v_i$ correspond to the uv-coordinate of the 3D body joint projected in the fisheye image space, and $d_i$ denotes the distance of the joint to the fisheye camera. Finally, the 3D body joints $\mathbf{\hat{J}}_b=\{(x_i, y_i, z_i) \mid i\in 0, 1, 2,..., J\}$ are recovered with the fisheye reprojection function: $(x_i, y_i, z_i) = \mathcal{P}^{-1}(u_i, v_i, d_i)$. The predicted body pose $\mathbf{\hat{J}}_b$ is finally compared with the ground truth body pose $\mathbf{J}_{b}$ with the MSE loss. \JW{We prove that the heatmap can also be used under the fisheye setup. To ensure the pixel-align feature, we apply the transformation on the extracted pose.}

Our proposed pixel-aligned heatmap representation solves problems in all three types of previous egocentric joint regressors. 
First, Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} employs separate networks to predict 2D joint positions and joint distances. However, this method can yield unrealistic joint estimations because small errors in 2D joints can result in large errors in 3D joints due to the projection effect. 
Second, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} and EgoHMR~\cite{liu2023egohmr} directly regress the 3D joint positions. However, this method is agnostic to the fisheye camera parameters, making it suitable only for a specific camera configuration (\eg, camera parameters, head-mounted position, \etc). 
Third, SceneEgo~\cite{wang2023scene} projects 2D features into 3D voxel space and uses a V2V network to regress 3D poses. Because of these, the SceneEgo method suffers from low accuracy and large computation overhead.
% Our pixel-aligned 3D heatmap stands out for its accuracy, simplicity, and speed. 
Different from the previous, Our pixel-aligned 3D heatmap directly estimates 3D joints while also incorporating an explicitly parametrized fisheye camera model. 
% This approach provides a more versatile and efficient solution to tackle the challenges in egocentric pose estimation. 
Moreover, it can preserve the uncertainty of the estimated joints, which will be used in our uncertainty-aware motion refinement method (Sec.~\ref{method:uncertainty_aware}). Detailed comparison with other pose prediction heads is shown in Table~\ref{table:ablation_study}.

% Our proposed pixel-aligned heatmap representation solves problems in all three types of previous egocentric joint regressors. 
% First, Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} employs separate networks to predict 2D joint positions and joint distances and then calculates 3D joint positions using a fisheye reprojection function. However, this method can yield unrealistic joint estimations because small errors in 2D joints can result in large errors in 3D joints due to the projection effect. 
% Second, $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} and EgoHMR~\cite{liu2023egohmr} directly regress the 3D joint positions. However, this method is agnostic to the fisheye camera parameters, making it suitable only for a specific camera configuration (\eg, camera distortion parameters, focal length, head-mounted position, \etc). 
% Third, SceneEgo~\cite{wang2023scene} projects 2D features into 3D voxel space with the fisheye reprojection function and uses a V2V network to regress 3D joints. However, this method suffers from low training and inference speed and large memory consumption, mainly because of the V2V network. In contrast to the above methods, our pixel-aligned 3D heatmap stands out for its simplicity and speed. It directly estimates 3D joints while also incorporating an explicitly parametrized fisheye camera model. This approach provides a more versatile and efficient solution to tackle the challenges in egocentric pose estimation. Moreover, it can preserve the uncertainty of the estimated joints, which will be used in our uncertainty-aware motion refinement method (Sec.~\ref{method:uncertainty_aware}). Detailed comparison with other pose prediction heads is shown in Table~\ref{table:ablation_study}.

\subsubsection{Egocentric Hand Pose Estimation} \label{method:wholebodypose}

In this section, we first train a network to detect hand pose locations and then train a 3D hand pose estimation network to regress 3D hand poses. Then, we describe how to integrate the estimated hand and body poses.

\noindent\textbf{Hand Detection.}
Given an input image $\mathbf{I}$, we finetune the ViTPose~\cite{xu2022vitpose} network to regress the 2D hand poses of left hand $\mathbf{J}^{2d}_{lh}$ and right hand $\mathbf{J}^{2d}_{rh}$. From the 2D hand poses, we obtain the center point of left hand $\mathbf{C}_{lh}$ and right hand $\mathbf{C}_{rh}$, along with the bounding box sizes, $d_{lh}$ and $d_{rh}$ for the 2D hand poses. We use our approach described in Sec.~\ref{method:fisheyevit} to compute undistorted image patches of left $\mathbf{I}_{lh}$ and right hands $\mathbf{I}_{rh}$.

\noindent\textbf{Hand Pose Estimation.}
Given the cropped image $\mathbf{I}_{lh}$ or $\mathbf{I}_{rh}$, we regress the 3D hand poses $\mathbf{\hat{J}}^{loc}_{lh}$ and $\mathbf{\hat{J}}^{loc}_{rh}$ with the Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} network, which is fine-tuned on our EgoFullBody dataset.

\noindent\textbf{Integration of Body and Hand Poses.}
It is not straightforward to integrate the hand poses with the body pose in the egocentric camera view primarily due to the fisheye camera's perspective effects. Take the left hand as an example. Following Step 3 in Sec.~\ref{method:fisheyevit}, we establish a local coordinate system on the tangent plane of the left-hand image with XYZ axes as follows: $x: \mathbf{v}^x_{lh}$; $y: \mathbf{v}^y_{lh}$; $z: \mathbf{v}^z_{lh}$. We define a rotation matrix, denoted as $\mathbf{R}$, that represents the transformation between the root coordinate system and the local coordinate system on the tangent plane. The estimated hand pose is first rotated with the rotation matrix $\mathbf{\hat{J}}_{lh} = \mathbf{R}\mathbf{\hat{J}}^{loc}_{lh}$ and then translated to align the wrist location of the human body. This same process is also applied to the right hand to get the right hand pose $\mathbf{\hat{J}}_{rh}$. The whole-body joints $\mathbf{\hat{J}}$ are obtained by combining $\mathbf{\hat{J}}_{b}$,  $\mathbf{\hat{J}}_{lh}$, and $\mathbf{\hat{J}}_{rh}$. The uncertainty of whole-body joints $\mathbf{\hat{U}}$ is also obtained from the maximal value of the 3D heatmap in pose estimation modules.

\subsection{Diffusion-Based Motion Refinement} \label{method:diffusion}

We notice that the single-frame estimations in Sec.~\ref{method:single_image_pose} suffer from inaccuracies and temporal instabilities. In this section, we propose a diffusion-based motion refinement method to tackle this problem. We first learn the whole-body motion prior with the motion diffusion model in Sec.~\ref{method:wholebody_motion_diffusion} and then introduce an uncertainty-aware zero-shot motion refinement method in Sec.~\ref{method:uncertainty_aware}.

\subsubsection{Whole-Body Motion Diffusion Model} \label{method:wholebody_motion_diffusion}

% We introduce our whole-body motion encoding, represented as $\mathbf{x}$, which relies on the sequence of whole-body joints. Each whole-body joint $\mathbf{J}$ in the sequence is adjusted to its original position and aligned to face forward. Hand joints and body joints are separated and individually normalized. The root orientation and root velocity are combined with the normalized hand and body joints. This combined information is stacked frame by frame, resulting in the whole-body motion encoding $\mathbf{x}$.

We follow DDPM~\cite{ho2020denoising} as our diffusion approach to capture the whole-body motion prior $q(\mathbf{x})$. DDPM learns a distribution of whole-body motion $\mathbf{x}$ through a forward diffusion process and an inverse denoising process. 
The forward diffusion process is a Markov process of adding Gaussian noise over $t \in \{0, 1, ..., T-1\}$ steps:
\begin{equation}
    q(\mathbf{x}_t|\mathbf{x}_{t-1}) = \mathcal{N}(\sqrt{\alpha_t}\mathbf{x}_{t-1}, (1 - \alpha_t)I)
\end{equation}
where $\mathbf{x}_t$ denotes the whole-body motion sequence at step $t$, the variance $(1-\alpha_t) \in (0, 1]$ denotes a constant hyperparameter increases with $t$. 

The inverse process uses a denoising network $D(\cdot)$ to remove the added Gaussian noise at each time step $t$. Here we use the transformer-based framework in EDGE~\cite{tseng2023edge} as the motion-denoising network $D(\cdot)$. We follow Ramesh~\etal's work~\cite{ramesh2022hierarchical} to make the network predict the original signal itself, \ie $\mathbf{\hat{x}}_0 = D(\mathbf{x}_t, t)$ and train it with the simple objective~\cite{ho2020denoising}:
\begin{equation}
    \mathcal{L}_{\text{simple}} = E_{\mathbf{x}_0 \sim q(\mathbf{x}_0), t \sim [1, T]}\left[ \vert\vert\mathbf{x}_0 - D(\mathbf{x}_t, t)\vert\vert^2_2 \right]
\end{equation}


\subsubsection{Uncertainty-Aware Motion Refinement} \label{method:uncertainty_aware}

Given the learned whole-body motion prior, we leverage the uncertainty value for each pose to guide the diffusion denoising process with the classifier-guided diffusion sampling~\cite{dhariwal2021diffusion}. Given an initial sequence of whole-body pose estimation $\mathbf{x}_e = \{\mathbf{\hat{J}}_i\}$ and the uncertainty value for each pose $\mathbf{u} = \{\mathbf{\hat{U}}_i\}$, where $i$ denotes the $i$th pose in the sequence, we keep the joints with low uncertainty but use the diffusion model to generate joints with high uncertainty conditioned on the low-uncertainty joints. Specifically, in the $t$th sampling step of the diffusion process, the denoising network predicts $\mathbf{\hat{x}}_0 = D(\mathbf{x}_t, t)$, which is noised back to $\mathbf{x}_{t-1}$ by sampling from the Gaussian distribution:
% \begin{equation}
% \begin{split}
%     \mathbf{x}_{t-1} &\sim \mathcal{N}(\mathbf{\hat{x}}_0 + w(\mathbf{x}_e - \mathbf{\hat{x}}_0), \Sigma_t); \\
%     w &= (1 + \exp(-k(t-T\mathbf{u}_e)))^{-1}
% \end{split}
% \end{equation}
\begin{equation}
    \mathbf{x}_{t-1} \sim \mathcal{N}(\mathbf{\hat{x}}_0 + \mathbf{w}(\mathbf{x}_e - \mathbf{\hat{x}}_0), \Sigma_t)
\end{equation}
where $\Sigma_t$ is a scheduled Gaussian distribution in DDPM~\cite{ho2020denoising} and $\mathbf{w}$ controls the weight of a specific joint between the predicted motion $\mathbf{\hat{x}}_0$ and the estimated motion $\mathbf{x}_e$. Generally, we expect $\mathbf{w} \rightarrow \overrightarrow{0}$ when $t \rightarrow 0$ such that the temporal stability is guaranteed through the generation of the denoising process, and $\mathbf{w} \rightarrow \overrightarrow{1}$ when $t \rightarrow T$ such that the denoising process is initialized by the estimated motion $\mathbf{x}_e$. We also expect that $w_{ij} = \mathbf{w}[i][j]$, which is the weight of $j$th joints in the $i$th pose, is smaller when the uncertainty value $u_{ij} = \mathbf{u}[i][j]$ of the $j$th joints in the $i$th pose is large. Based on this requirement, we design $\mathbf{w}$ as:
\begin{equation}
    \mathbf{w} = 1 / \left(1 + e^{-k(t-T\mathbf{u})}\right)
\end{equation}
where $T$ is the overall diffusion steps, $k$ is a hyperparameter which is empirically set to $0.1$.
% \ZC{perhaps need to add ablations of different $\mathbf{w}$ function choices in the supplement} 
From the experimental results in Sec.~\ref{experiments}, we demonstrate the effectiveness of uncertain-aware motion refinement and our uncertainty-guided diffusion sampling strategy.


\section{EgoWholeMocap Dataset} \label{method:synthetic_dataset}

In this section, we introduce EgoWholeMocap, a large-scale high-quality synthetic dataset built for the task of egocentric whole-body motion capture. The EgoWholeMocap dataset is organized into two sections. The first part, containing over 700k frames, is rendered with 14 different rigged Renderpeople~\cite{renderpeople} models driven by 2367 Mixamo~\cite{mixamo} motion sequences. Note that the Mixamo~\cite{mixamo} motions used in this part mainly focus on body movements, lacking diversity in hand motions. The second part of our dataset focuses on more complex hand motions and contains 170k frames with the SMPL-X model. This data is constructed from 24 different shapes and textures, driven by 200 motion sequences selected from the GRAB dataset~\cite{taheri2020grab} and 62 motion sequences from the TCDHandMocap dataset~\cite{hoyet2012sleight}. 

During the rendering process, we first attach a virtual fisheye camera to the forehead of human body models and render the images, semantic labels, and depth map with Blender~\cite{blender}. 
% The EgoWholeMocap dataset offers a valuable resource for advancing research in egocentric whole-body motion capture. 
Our dataset is larger and more diverse than previous egocentric training datasets--see Sec.~\ref{supp:dataset_comparison} in the supplementary material for a detailed comparison. 
% \DL{I suggest that we make the paragraph in the intro about the dataset L085-L097 more high level, without giving too much details about each dataset used, and place these two last sentences from here there, to emphasize that our dataset is a valuable contribution.}

==> sec/bak/4_experiments_bak.tex <==
\section{Experiments} \label{experiments}

\begin{figure*}
\centering
\includegraphics[width=0.99\linewidth]{fig/results/results_body_crop.pdf}
\caption{Qualitative comparison on human body pose estimations between our methods and the state-of-the-art egocentric pose estimation methods on in-the-studio (left column) and in-the-wild scenes (right column). The red skeleton is the ground truth while the green skeleton is the predicted pose. Our methods predict more accurate body poses compared with EgoPW~\cite{Wang_2022_CVPR} and SceneEgo~\cite{wang2023scene}.
\vspace{-1em}
}
\label{fig:results}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.99\linewidth]{fig/results/results_hand_crop.pdf}
\caption{Qualitative comparison on human hand pose estimations between our methods and the state-of-the-art third-view pose estimation methods. Our single-view and refined hand poses are more accurate than the poses from Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} method. The red skeleton is the ground truth while the green skeleton is the predicted pose. 
\vspace{-1em}
}
\label{fig:results_hand}
\end{figure*}

\subsection{Datasets and Evaluation Metrics}

\noindent\textbf{Training Datasets.} \label{dataset:training}
To train our body pose estimation module (Sec.~\ref{method:fisheyevit} and Sec.~\ref{method:pixel_aligned_heatmap}), we use our EgoWholeBody dataset and the EgoPW dataset~\cite{wang2021estimating}. 
% The EgoPW dataset is an in-the-wild dataset containing 65k images annotated with the pseudo-ground truth. 
Additionally, the EgoWholeBody dataset is used to train the hand pose estimation module in Sec.~\ref{method:wholebodypose}.
% To train our human body pose estimation networks (FisheyeViT + pixel-aligned 3D heatmap), we initialize the transformer in FisheyeViT with VitPose~\cite{xu2022vitpose}. Subsequently, we train the network using our EgoWholeBody dataset and the EgoPW dataset~\cite{wang2021estimating}. The same EgoWholeBody dataset is also utilized for training the hand detection and hand pose estimation network. 
For training the whole-body diffusion model (Sec.~\ref{method:diffusion}), we utilize a combined motion capture dataset that includes EgoBody~\cite{zhang2022egobody}, Mixamo~\cite{mixamo}, TCDHandMocap dataset~\cite{hoyet2012sleight} and GRAB dataset~\cite{taheri2020grab}.

\noindent\textbf{Evaluation Datasets.} 
In our experiment, we evaluate our methods on three datasets: the GlobalEgoMocap test datasets~\cite{wang2021estimating}, the Mo$^2$Cap$^2$ test dataset~\cite{DBLP:journals/tvcg/XuCZRFST19} and the SceneEgo test dataset~\cite{wang2023scene}. The details of these datasets are shown in Sec.~\ref{supp:evaluation_dataset} of supplementary materials. 
% We notice that evaluating whole-body poses requires accurate annotations for human hands and body. Unfortunately, the aforementioned evaluation datasets lack hand annotations. To solve this, we used a multi-view motion capture system to capture the hand motion in the SceneEgo test dataset~\cite{wang2023scene}. The hand pose annotations will be made public.
Note that evaluating whole-body poses requires accurate annotations for human hands, which is absent in these datasets. To resolve the issue, we request the multi-view videos of the SceneEgo test dataset~\cite{wang2023scene} from the authors and use a multi-view motion capture system to obtain the hand motion. The hand pose annotations will be made public.

\noindent\textbf{Evaluation Metrics.}
To evaluate the precision of human body poses on the SceneEgo test dataset~\cite{wang2023scene}, we use MPJPE and PA-MPJPE. For the GlobalEgoMocap test dataset~\cite{wang2021estimating} and Mo$^2$Cap$^2$ test dataset~\cite{DBLP:journals/tvcg/XuCZRFST19}, where egocentric camera poses are unavailable, we evaluate PA-MPJPE and BA-MPJPE.
For hand pose accuracy, we align the predicted and ground truth hand poses at the root position, followed by computing MPJPE and PA-MPJPE. Detailed explanations of these metrics are in Sec.~\ref{supp:evaluation_metrics} of the supplementary materials. All reported metrics are in millimeters.

\subsection{Comparisons on Whole-Body Pose Estimation} \label{experiments:main_comparison}

% In this section, we first compare the body pose estimation result from our method (without using diffusion-based refinement) and the results from state-of-the-art egocentric body pose estimation methods, EgoPW~\cite{Wang_2022_CVPR}, SceneEgo~\cite{wang2023scene}, EgoHMR~\cite{liu2023egohmr} and Ego-STAN~\cite{park2023domain}. Results are presented in Table~\ref{table:main}, with our result labeled as ``Ours-Single''. Across all three evaluation datasets, our single-frame method consistently outperforms all previous methods with a large margin in terms of body pose estimation accuracy.

In this section, we first compare our single-frame body pose estimation result (w/o diffusion-based refinement) with state-of-the-art egocentric body pose estimation methods: EgoPW~\cite{Wang_2022_CVPR}, SceneEgo~\cite{wang2023scene}, EgoHMR~\cite{liu2023egohmr} and Ego-STAN~\cite{park2023domain}. Results are presented in Table~\ref{table:main}, with our result labeled as ``Ours-Single''. Across all three evaluation datasets, our single-frame method consistently outperforms all previous methods by a large margin.
% in terms of body pose estimation accuracy.

To evaluate the accuracy of our hand pose estimation method, we first crop the hand images with the hand detection method in Sec.~\ref{method:wholebodypose}. We compare with~\cite{Moon_2022_CVPRW_Hand4Whole} and report the accuracy of estimated hand poses on the SceneEgo test set in Table~\ref{table:hand}. The result indicates that our method outperforms the baseline hand pose estimation method, Hands4Whole~\cite{Moon_2022_CVPRW_Hand4Whole}, which is one of the state-of-the-art third-view hand pose estimation methods.

We also evaluated our diffusion-based whole-body motion refinement method in Table~\ref{table:main}. Since our motion refinement method incorporates random Gaussian noise, we generate five samples and calculate the average MPJPE values. The standard deviation of the results is low ($<$ 0.01mm) and is discussed in Sec.~\ref{supp:std} of supplementary materials. As shown in Table~\ref{table:main} and Table~\ref{table:hand}, the diffusion-based motion refinement method, denoted as ``Ours-Refined'', enhances the accuracy of the estimated whole-body motion. The human body MPJPE is better than our single-frame method by 8.2\% while hand MPJPE is better than our single-frame method by 18.0\% on the SceneEgo test dataset. 

For a qualitative comparison, we compare the human body and hand poses of our method with existing methods on the SceneEgo dataset and in-the-wild sequences from the EgoPW evaluation sequence. The results are shown in Fig.~\ref{fig:results} and Fig.~\ref{fig:results_hand}. Please refer to our supplementary video for more qualitative evaluation results.

We observe that previous methods~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19, wang2021estimating, Wang_2022_CVPR, wang2023scene} use training datasets different from each other. To ensure a fair comparison in body pose estimation methods, we re-train previous methods with our training datasets in Sec.~\ref{dataset:training} and show the results in Sec.~\ref{supp:full_comparison} of the supplementary materials.

\begin{table}
\begin{center}
\small
\begin{tabularx}{0.47\textwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X  }
\hlineB{2.5}
Method & MPJPE & PA-MPJPE \\
\hline
\multicolumn{2}{l}{\textbf{SceneEgo test dataset~\cite{wang2023scene}}} \\
\hline
EgoPW~\cite{Wang_2022_CVPR} & 189.6 & 105.3 \\
SceneEgo~\cite{wang2023scene} & 118.5 & 92.75 \\
\hline
Ours-Single & \underline{64.19} & \underline{50.06} \\
% Ours-Refined$^\dagger$ & \textbf{57.59$\pm$0.003} & \textbf{46.55$\pm$0.003} \\
Ours-Refined$^\dagger$ & \textbf{57.59} & \textbf{46.55} \\
\hlineB{2.5}
Method & PA-MPJPE & BA-MPJPE \\
\hline
\multicolumn{2}{l}{\textbf{GlobalEgoMocap test dataset~\cite{wang2021estimating}}} \\
\hline
EgoPW~\cite{Wang_2022_CVPR} & 81.71 & 64.87 \\
EgoHMR~\cite{liu2023egohmr} & 85.80 & -- \\
SceneEgo~\cite{wang2023scene} & 76.50 & 61.92 \\
\hline
Ours-Single & \underline{68.59} & \underline{55.92} \\
% Ours-Refined$^\dagger$ & \textbf{65.83$\pm$0.003} & \textbf{53.47$\pm$0.003} \\
Ours-Refined$^\dagger$ & \textbf{65.83} & \textbf{53.47} \\
\hlineB{2.5}
\multicolumn{2}{l}{\textbf{Mo$^2$Cap$^2$ test dataset~\cite{DBLP:journals/tvcg/XuCZRFST19}}} \\
\hline
EgoPW~\cite{Wang_2022_CVPR} & 83.17 & 64.33 \\
Ego-STAN$^\dagger$~\cite{park2023domain} & 102.4 & -- \\
SceneEgo~\cite{wang2023scene} & 79.65 & 62.82 \\
\hline
Ours-Single & \underline{74.66} & \underline{59.26} \\
% Ours-Refined$^\dagger$ & \textbf{72.63$\pm$0.003} & \textbf{57.12$\pm$0.003} \\
Ours-Refined$^\dagger$ & \textbf{72.63} & \textbf{57.12} \\
\hlineB{2.5}
\end{tabularx}
\end{center}
\vspace{-1em}
\caption{
Egocentric human body pose accuracy of our method on three test datasets. Our method outperforms all previous state-of-the-art methods. $^\dagger$ denotes the temporal-based methods. 
% Our method also outperforms a video-based method~\cite{wang2021estimating} in terms of  PA-MPJPE.
}
\vspace{-0.5em}
\label{table:main}
\end{table}

\begin{table}
\begin{center}
\small
\begin{tabularx}{0.47\textwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X  }
\hlineB{2.5}
Method & MPJPE & PA-MPJPE \\
\hline
Hand4Whole~\cite{Moon_2022_CVPRW_Hand4Whole} & 49.66 & 13.85 \\
Ours-Single & 23.63 & 9.59 \\
% Ours-Refined & \textbf{19.37$\pm$0.003} & \textbf{9.05$\pm$0.003} \\
Ours-Refined & \textbf{19.37} & \textbf{9.05} \\
\hlineB{2.5}
\end{tabularx}
\end{center}
\vspace{-1em}
\caption{Egocentric hand pose accuracy of our method on SceneEgo test dataset. Our method outperforms the state-of-the-art Hand4Whole method~\cite{Moon_2022_CVPRW_Hand4Whole}. 
\vspace{-0.5em}
}
\label{table:hand}
\end{table}

\subsection{Ablation Study} \label{ablation_study}


\begin{table}
\begin{center}
\small
\begin{tabularx}{0.47\textwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash\hsize=.5\hsize}X 
   >{\centering\arraybackslash\hsize=.5\hsize}X  }
\hlineB{2.5}
Method & MPJPE & PA-MPJPE \\
\hline
\multicolumn{2}{l}{\textbf{Body Pose Results}} \\
\hline
w/o EgoWholeBody data  & 75.10 & 58.62 \\
w/o FisheyeViT  & 67.36 & 53.44 \\
% w/o PA-HM  & 125.7 & 90.48 \\
w/ Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} head  & 87.47 & 65.10 \\
% w/ Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} head  & 96.13 & 72.39 \\
w/ $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} head  & 116.5 & 95.78 \\
w/ SceneEgo~\cite{wang2023scene} head  & 77.73 & 62.69 \\
% w/ SceneEgo~\cite{wang2023scene} head  & 87.33 & 64.51 \\
Ours-Single & \textbf{64.19} & \textbf{50.06} \\
\hline
w/ GlobalEgoMocap$^\dagger$ & 69.83 & 56.73 \\
% w/ Gaussian Smooth$^\dagger$ & 62.68 & 48.87 \\
w/o uncert. guidance$^\dagger$ & 62.16 & 48.40 \\
Only body diffusion & 58.95 & 47.03 \\
Ours-Refined$^\dagger$ & \textbf{57.59}  & \textbf{46.55} \\
\hline
\multicolumn{2}{l}{\textbf{Hand Pose Results}} \\
\hline
% Only hand diffusion & 21.69$\pm$0.003 & 9.24$\pm$0.003 \\
Only hand diffusion & 21.69 & 9.24 \\
% Ours-Refined & \textbf{19.37$\pm$0.003}  & \textbf{9.05$\pm$0.003} \\
Ours-Refined & \textbf{19.37}  & \textbf{9.05} \\
\hlineB{2.5}
\end{tabularx}
\end{center}
\vspace{-1em}
\caption{Ablation Study on SceneEgo test dataset~\cite{wang2023scene}. 
% about the single-frame method and diffusion-based motion refinement. 
$^\dagger$ denotes the temporal-based method.
\vspace{-0.5em}
}
\label{table:ablation_study}
\end{table}

\noindent\textbf{EgoWholeBody Dataset.}
Compared to existing egocentric datasets, our EgoWholeBody dataset contains diverse body motion and hand motion, larger quantity of images, and higher image quality. We demonstrate this by training our body pose estimation network without our dataset, using the Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and EgoPW~\cite{Wang_2022_CVPR} training dataset. The results, labeled as "w/o EgoWholeBody Data" in Table~\ref{table:ablation_study}, show that performance without the EgoWholeBody dataset is inferior to our proposed method. This highlights that training with our high-quality EgoWholeBody dataset enhances the performance of the pose estimation method.
% This highlights that training with the high-quality synthetic EgoWholeBody dataset enhances the performance of our single-frame pose estimation method.


\noindent\textbf{FisheyeViT and Pixel-Aligned Heatmap.}
To assess the individual contributions of FisheyeViT and the pixel-aligned 3D heatmap in our single-frame pose estimation pipeline, we perform experiments to measure their impact on the overall performance. First, we substitute the FisheyeViT module in our single-frame pose estimation method to ViT~\cite{dosovitskiy2020image}. The result is shown in ``w/o FisheyeViT'' in Table~\ref{table:ablation_study} and it is worse than our full method. This demonstrates the effectiveness of FisheyeViT in addressing fisheye distortion and feature extraction. 

Next, we analyze the performance of the single-frame pose estimation network when substituting the pixel-aligned 3D heatmap with the pose estimation heads of previous works~\cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19, wang2023scene}. The results of the three experiments, labeled as ``w/ Mo$^2$Cap$^2$ head'', ``w/ $x$R-egopose head'' and ``w/ SceneEgo head'', show a performance drop compared to our full method. This emphasizes the crucial role of the pixel-aligned 3D heatmap in accurately estimating egocentric 3D body joint positions.

\noindent\textbf{Diffusion-based Motion Refinement.}
In this ablation study, we assess the effectiveness of our diffusion-based motion refinement with the following experiments: 

First, we compare the performance of our diffusion-based motion refinement with GlobalEgoMocap~\cite{wang2021estimating} by applying the GlobalEgoMocap optimizer on the single-frame body pose estimation results. The result, labeled as ``w GlobalEgoMocap'' in Table~\ref{table:ablation_study}, indicates that our refinement method outperforms GlobalEgoMocap, demonstrating the effectiveness of our diffusion-based motion refinement. 

% Second, we tested our method against a simpler one using Gaussian smoothness to refine the initial whole-body poses. The results labeled ``w Gaussian Smooth'' in Table~\ref{table:ablation_study} demonstrate that our method performed better. Our diffusion-based refinement relies on motion priors to guide the refinement of human motion, making it more effective than simple smoothing methods.

Second, we remove the uncertainty-aware guidance in the motion refinement. Instead, we first add Gaussian noise for $t$ steps, then use the denoising process to generate the clean whole-body motion. Here we set $t=5$ for the best result. The result, labeled as ``w/o uncert. guidance'' in Table~3, shows that our uncertainty-aware refinement method performs better. Our approach relies on the uncertainty values for each joint, using low-uncertainty joints to guide the generation of high-uncertainty joints. This helps reduce errors in joint predictions caused by egocentric self-occlusion, leading to improved results.

% \noindent\textbf{Whole-Body Motion Refinement}
Third, 
% in our method, we introduce the whole-body motion diffusion model to capture the whole-body motion prior, including the correlation between the human body and hand motion. In this experiment, 
we replace our whole-body motion diffusion model with the separate human body and left/right-hand diffusion models and show the accuracy of refined body and hand motion in ``Only body diffusion'' and ``Only hand diffusion'' in Table~\ref{table:ablation_study}. From the results, we observe improvements in the accuracy of motion refined by our whole-body diffusion method, proving that learning the whole-body motion prior can help both the refinement of the human body and hand motion by learning the correlation between the human body and hand motion.
% \begin{table}
% \begin{center}
% \small
% \begin{tabularx}{0.47\textwidth} { 
%    >{\raggedright\arraybackslash}X 
%    >{\centering\arraybackslash\hsize=.5\hsize}X 
%    >{\centering\arraybackslash\hsize=.5\hsize}X  }
% \hlineB{2.5}
% Method & MPJPE & PA-MPJPE \\
% \hline
% Only body diffusion & 58.95$\pm$0.05 & 47.03$\pm$0.05 \\
% Our body poses acc. & \textbf{57.59$\pm$0.05}  & \textbf{46.55$\pm$0.05} \\
% \hline
% Only hand diffusion & 21.69$\pm$0.04 & 9.24$\pm$0.04 \\
% Our hand poses acc. & \textbf{19.37$\pm$0.04}  & \textbf{9.05$\pm$0.04} \\
% \hlineB{2.5}
% \end{tabularx}
% \end{center}
% \vspace{-1em}
% \caption{Ablation Study on the whole-body diffusion model.
% \vspace{-0.5em}
% }
% \label{table:ablation_whole_body_diffusion}
% \end{table}

